Trust the uncertain teacher: distilling dark knowledge via calibrated uncertainty

The core of knowledge distillation lies in transferring the teacher's rich 'dark knowledge'-subtle probabilistic patterns that reveal how classes are related and the distribution of uncertainties. While this idea is well established, teachers trained with conventional cross-entropy often fail to preserve such signals. Their distributions collapse into sharp, overconfident peaks that appear decisive but are in fact brittle, offering little beyond the hard label or subtly hindering representation-level transfer. This overconfidence is especially problematic in high-cardinality tasks, where the nuances among many plausible classes matter most for guiding a compact student. Moreover, such brittle targets reduce robustness under distribution shift, leaving students vulnerable to miscalibration in real-world conditions. To address this limitation, we revisit distillation from a distributional perspective and propose Calibrated Uncertainty Distillation (CUD), a framework designed to make dark knowledge more faithfully accessible. Instead of uncritically adopting the teacher's overconfidence, CUD encourages teachers to reveal uncertainty where it is informative and guides students to learn from targets that are calibrated rather than sharpened certainty. By directly shaping the teacher's predictive distribution before transfer, our approach balances accuracy and calibration, allowing students to benefit from both confident signals on easy cases and structured uncertainty on hard ones. Across diverse benchmarks, CUD yields students that are not only more accurate, but also more calibrated under shift and more reliable on ambiguous, long-tail inputs.

==> iclr2026/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> iclr2026/sections/00_abstract.tex <==

\begin{abstract}
본 논문에서는 knowledge distillation(KD) 성능 향상을 위해, 모델의 응답을 기반으로 오답에 집중적으로 학습하여 distillation에 적합한 teacher를 구축하고, 오답 전이를 억제하면서 클래스 간 관계 정보를 효과적으로 전달할 수 있는 새로운 distillation 전략을 제안한다. 최근 대규모 언어 모델(LLM)의 상용화를 위한 모델 압축 기법으로 pruning, quantization, KD 등이 활발히 연구되고 있으며, 그중 KD는 teacher의 지식을 student 모델로 전이하는 핵심 기법으로 주목받고 있다. 기존 KD 연구들은 teacher의 representation이나 attention score 등 다양한 정보를 활용하여 loss term을 설계하지만, 지식의 신뢰도와 무관하게 무조건적으로 전이한다는 한계가 존재한다. 이를 개선하기 위해, 본 연구에서는 teacher가 정답을 쉽게 예측하는 경우 학습 비중을 낮추고, 오답이거나 불확실성이 큰 경우에는 학습을 강화하는 전략을 적용하였다. 또한, teacher의 오답이 student로 그대로 전이되는 것을 방지하면서도 클래스 간 관계 정보를 보존할 수 있는 새로운 distillation 방법을 제안한다. BERT를 활용한 다중 분류 태스크 및 GLUE 실험 결과, 제안 방법은 단순 fine-tuned 모델 대비 절대 정확도는 일부 낮을 수 있으나, distillation 성능 측면에서는 기존 접근법보다 우수함을 실험적으로 확인하였다.
\end{abstract}

==> iclr2026/sections/00_abstract_en.tex <==
\begin{abstract}

The core of knowledge distillation lies in transferring the teacher's rich `\textit{dark knowledge}'—subtle probabilistic patterns that reveal how classes are related and the distribution of uncertainties.
While this idea is well established, teachers trained with conventional cross-entropy often fail to preserve such signals.
Their distributions collapse into sharp, overconfident peaks that appear decisive but are in fact brittle, offering little beyond the hard label or subtly hindering representation-level transfer.
This overconfidence is especially problematic in high-cardinality tasks, where the nuances among many plausible classes matter most for guiding a compact student. 
Moreover, such brittle targets reduce robustness under distribution shift, leaving students vulnerable to miscalibration in real-world conditions.
To address this limitation, we revisit distillation from a distributional perspective and propose Calibrated Uncertainty Distillation (CUD), a framework designed to make dark knowledge more faithfully accessible.
Instead of uncritically adopting the teacher’s overconfidence, CUD encourages teachers to reveal uncertainty where it is informative and guides students to learn from targets that are calibrated rather than sharpened certainty.
By directly shaping the teacher’s predictive distribution before transfer, our approach balances accuracy and calibration, allowing students to benefit from both confident signals on easy cases and structured uncertainty on hard ones.
Across diverse benchmarks, CUD yields students that are not only more accurate, but also more calibrated under shift and more reliable on ambiguous, long-tail inputs.
% Beyond improving accuracy, CUD contributes a principled view of knowledge transfer as preserving distributional structure, positioning distillation as not just compression but a tool for robust uncertainty propagation.
\end{abstract}


==> iclr2026/sections/01_intro.tex <==

\section{Introduction}
최근 대규모 언어 모델(LLM; e.g., GPT-4 \cite{openai2023gpt4}, PaLM \cite{chowdhery2022palm}, LLaMA \cite{touvron2023llama}, Gemini \cite{gemini2023})의 급격한 발전은 자연어 처리(NLP)와 다양한 인공지능 응용 분야에서 혁신적인 성과를 이끌어내고 있다. 이러한 모델들은 기계 번역, 문서 요약, 대화형 에이전트, 코드 생성 등 다양한 작업에서 기존의 방법론을 뛰어넘는 성능을 보여주며 활용 방안을 확장시킨다. 그러나 모델 규모가 수십억~수천억 개의 파라미터에 달하면서 모델을 실제로 활용함에 있어서 높은 연산 비용과 메모리 제약이 발생한다는 한계가 존재한다.

이러한 제약을 해결하기 위해 모델 압축(model compression) 및 경량화(lightweighting) 기법들이 활발히 연구되고 있다. 대표적으로 quantization \cite{hubara2017quantized}, pruning \cite{han2015efficient}, low-rank adaptation (LoRA) \cite{hu2022lora}와 같은 parameter-efficient fine-tuning (PEFT) 기법이 있다. 이 중 Knowledge Distillation (KD) \cite{hinton2015distilling}은 대규모 teacher 모델의 지식을 소규모 student 모델에 효과적으로 전달하여, 작은 모델이 적은 학습 비용만으로도 우수한 성능을 달성할 수 있도록 하는 강력한 모델 경량화 방법으로 자리 잡고 있다. 본 논문은 KD에 초점을 맞추어, 통상적인 방식으로 학습한 teacher 모델의 distillation에 있어서의 한계를 지적하고, distillation 친화적인 teacher를 위한 새로운 학습 전략을 제안한다.


\begin{figure}[h]
    \centering
    \includegraphics[width=0.7\textwidth]{figures/figure3.png} 
    \caption{우리 방법은 Teacher 모델을 학습할 때 focal–entropy loss를 적용하여, 정답 샘플에는 낮은 가중치를, 오답 샘플에는 높은 가중치를 부여함으로써 softened distribution을 생성한다. 이렇게 정제된 분포는 원래의 날카로운 분포보다 더 풍부한 정보를 제공하며, Post-processing 단계를 거쳐 최종적으로 Student 모델로 지식이 증류 된다.}
    \label{fig:pipeline}
\end{figure}


기존 KD 연구는 크게 세 가지 축으로 분류된다: (1) teacher의 출력 응답(response) 기반 전이 \cite{hinton2015distilling}, (2) 중간 feature representation 기반 전이 \cite{romero2015fitnets}, (3) 데이터 간 관계(relation) 기반 전이 \cite{passalis2018probabilistic}. 또한 confidence score나 entropy를 활용하여 난이도에 따라 학습 순서를 조절하는 curriculum learning 접근법 \cite{park2021student} 역시 제안된 바 있다. 이와 같이 기존 연구들은 주로 “teacher가 보유한 지식을 어떻게 student에 효과적으로 전달할 것인가”에 초점을 맞추어 발전해왔다.

그러나 이러한 접근들은 teacher가 가진 모든 정보가 student에게 무조건적으로 유용하다는 가정을 내포한다. 실제로 teacher는 성능 극대화된 모델을 사용하는 것이 일반저기지만, 교사 모델에서 생성된 오답이나 불필요하게 복잡한 표현, 과도하게 확신하는 경향성은 student 학습에 혼선을 줄 수 있다.


따라서 더 높은 성능을 가진 teacher를 사용하더라도 distillation된 student가 반드시 더 나은 성능을 보장하지는 않는다 \cite{cho2019efficacy}. 이는 teacher 학습의 일반적 목표(성능 극대화)와 KD의 목표(효과적 지식 전이) 사이의 근본적 간극(gap)에서 기인한다. 이러한 문제를 해결하기 위해 본 논문에서는 distillation 친화적인 teacher 학습 방식을 설게하고, teacher 출력을 가공·후처리하여 student 친화적 지식을 전달하는 방식을 제안한다.

\noindent\textbf{Dark knowledge를 충분히 가진 teacher의 정의 및 중요성 강조}
    
    Hinton et al. \cite{hinton2015distilling}는 teacher의 soft output 분포에 담긴 비정답 클래스 간의 확률적 정보가 student 학습에 유용함을 지적하며 이를 dark knowledge라 정의하였다. Dong et al. \cite{dong2024student}는,, distillation의 효과는 teacher의 dark knowledge가 진정한 레이블 분포(true label distribution)에 얼마나 잘 근사하는지에 크게 의존한다고 언급한다. 여기서 “진정한 레이블 분포”는 어떤 입력에 대해 정답(label)이 하나의 클래스(one-hot)만이 되는 것이 아니라, 여러 클래스에 대한 실제 확률적 가능성을 반영하는 분포이다.
    
\noindent\textbf{Soft distribution의 필요성 및 focal loss 기반 접근}
    
    이러한 dark knowledge를 충분히 갖춘 teacher를 얻기 위해서는 output의 분포가 “soft”해야 한다. 즉, teacher가 어떤 예제에 대해 확신이 지나치게 높으면 non-정답 클래스에 대한 정보(예: class 간 상관관계)가 소실된다. 이를 방지하기 위해 본 논문은 focal loss \cite{lin2017focal}를 teacher 학습에 도입한다. 구체적으로, teacher가 정답을 맞춘 경우에는 손실 기여도를 상대적으로 낮추고, 오답인 경우에는 더 크게 반영하여 학습의 집중도를 조절한다. 이렇게 하면 teacher가 정답 케이스에 과도하게 과적합되는 것을 막고, 확률 분포(entropy)를 soft하게 유지하면서 정답 이외의 클래스에 대한 정보와 클래스 간의 관계에 대한 정보까지 반영하도록 유도할 수 있다.
    

본 연구는 기존 KD 연구가 주로 teacher의 response, feature에 집중하며 내제된 지식을 어떻게 전달할지에 초점을 맞춘 것과 달리, teacher 자체를 distillation 친화적으로 학습한다는 점에서 차별성을 갖는다. 특히, (1) focal loss를 통해 정답과 오답에 대한 가중치를 조절하며 학습, (2) soft distribution 기반 dark knowledge 강화, (3) teacher의 오답 정보에 대한 후처리 전략을 결합함으로써  distillation에 최적화된 teacher 모델을 제안한다.

==> iclr2026/sections/01_intro_en.tex <==
\section{Introduction}

LLMs such as GPT-4 \citep{openai2023gpt4}, PaLM \citep{chowdhery2022palm}, LLaMA \citep{touvron2023llama}, and Gemini \citep{gemini2023} deliver state-of-the-art results across reasoning, dialogue, and code generation, yet they impose heavy latency, memory, and energy costs at inference time. 
Among compression techniques including pruning and quantization, knowledge distillation (KD) \citep{hinton2015distilling} remains uniquely attractive because it transfers a teacher’s \emph{predictive distribution}, not just argmax labels, thereby capturing inter-class structure, inductive biases, and task-dependent uncertainty that smaller models would not infer from hard labels alone\citep{huang2022knowledge, moslemi2024survey}. 
The central hypothesis of this work is that, when appropriately preserved and transferred, the teacher’s distribution better approximates the latent true label distribution over plausible classes \citep{dong2024student}, producing students that generalize more reliably.

However, conventional supervised training often yields over-confident teacher\citep{wei2022mitigating, el2025drowning} whose probabilities collapse onto a single class, suppressing precisely the soft structure that makes KD effective. 
Post-hoc temperature scaling, which adjusts prediction sharpness with a global scalar after training, only rescales logits and cannot recover information that was never represented or was erased by overfitting \citep{guo2017calibration}. 
Regularizers such as label smoothing and confidence penalties may reduce calibration error, yet they can also blur informative class-wise geometry that students should imitate \citep{muller2019does, pereyra2017regularizing}. 
Much of the KD literature compensates on the student side while keeping the teacher fixed, for example via KL matching with a fixed temperature, intermediate feature hints, or self-distillation  \citep{zhang2019byot, mobahi2020selfdistillation}. 
These strategies are valuable, but they neither prevent distribution collapse in the teacher nor selectively filter teacher errors during transfer, leaving performance on borderline and long-tail examples especially fragile.

We take a distributional perspective on KD and argue that two properties are jointly required for strong downstream students. 
First, the \emph{teacher} should retain informative uncertainty, allocating non-trivial probability mass to semantically related alternatives where the task is intrinsically ambiguous. 
Second, the \emph{transfer} should be calibrated so that the student imitates informative relations while attenuating misleading teacher peaks that arise from over-confidence or spurious correlations. 
Intuitively, KD works best when the teacher behaves like a well-calibrated Bayesian posterior on easy and hard inputs alike, and when the student is encouraged to inherit that calibrated structure rather than the teacher’s certainty alone.
We define these characteristics in problem formulation section.

This view aligns with the empirical regularities observed across the modalities. 
In fine-grained classification and language understanding, soft targets consistently improve sample efficiency by encoding \emph{relative} similarities between classes that hard labels cannot convey. 
When the data distribution shift, students distilled from calibrated teachers achieve lower expected calibration error and maintain more stable confidence on near-OOD inputs. This stability leads to improved selective prediction and more favorable accuracy–rejection trade-offs\citep{guo2017calibration, mishra2023knowledge}.
%Under distribution shift, models distilled from calibrated teachers exhibit a lower expected calibration error and more stable confidence on near-OOD examples, which translates into better selective prediction and accuracy–rejection trade-offs \citep{guo2017calibration}. 
In resource-constrained deployments, such as on-device assistants~\citep{chi2025adaptive} and retrieval-augmented pipelines where latency budgets are tight~\citep{jiang2025piperag}, students that inherit calibrated uncertainty achieve competitive accuracy while maintaining predictable confidence estimates, a property that downstream systems can exploit for routing, abstention, and cost-aware ensembling.

Our study operationalizes this distributional stance without relying on architectural tricks or task-specific heuristics. 
We focus on \emph{why} preserving and selectively transferring dark knowledge is necessary and \emph{when} it pays off, rather than on implementation details. 
Empirically, we show that students trained under this lens achieve higher accuracy at fixed compute, improved robustness on ambiguous and long-tail slices, and better probabilistic calibration. 
The results support the thesis that effective KD should prioritize calibrated structure over sharpened certainty, bringing the student closer to the true label distribution while avoiding the teacher’s pitfalls.



==> iclr2026/sections/02_prelim.tex <==
\section{Problem Formulation}
\label{sec:problem}

\subsection{Preliminaries and Limitations of Conventional KD}
Let $\mathcal{X}$ be the input space and $\mathcal{Y}=\{1,\dots,C\}$ the label set. A teacher model induces a predictive distribution $p_T(\cdot \mid x)\in\Delta^{C-1}$ for $x\in\mathcal{X}$, and a student model with parameters $\theta_S$ induces $p_S(\cdot \mid x;\theta_S)\in\Delta^{C-1}$. Conventional knowledge distillation (KD) trains the student to match the teacher (optionally combined with ground-truth supervision):
\begin{equation}
\label{eq:student}
\min_{\theta_S}\ \mathbb{E}_{x\sim(\mathcal{D})}\!\Big[
\mathcal{L}_{\mathrm{KD}}\big(p_S(\cdot\mid x;\theta_S),\,\tilde p_T(\cdot\mid x)\big)\Big]
\;+\;
\lambda\,\mathbb{E}_{(x,y)\sim\mathcal{D}}\!\big[\mathcal{L}_{\mathrm{CE}}\big(p_S(\cdot\mid x),y\big)\big],
\end{equation}
% where $\tilde p_T$ denotes a (possibly processed) teacher target and $\mathcal{D}$ is the labeled set. In practice, maximum-likelihood training often over-sharpens $p_T$, erasing relational ``dark knowledge'' and amplifying erroneous peaks that are then propagated to $p_S$.

where $\tilde p_T(\cdot\mid x)$ denotes the \emph{calibrated} teacher target (usually just a temperature scaled version of $p_T$), and $\mathcal{D}$ is the labeled set. 
In practice, however, maximum likelihood training often produces an over confident $p_T$, so that even such temperature scaled targets can remain over sharpened, erasing relational ``dark knowledge'' and amplifying erroneous peaks that are then propagated to $p_S$.

\subsection{Guiding Principles for Calibrated Distillation}
We posit that KD can be simultaneously \emph{robust} and \emph{informative} when the following conditions hold.

\paragraph{C1: Difficulty-aware uncertainty.}
For ambiguous or challenging inputs, the teacher should preserve uncertainty correspond to task difficulty rather than collapsing probability mass onto a single class. 
Concretely, the teacher should retain non-trivial probability on semantically related alternatives, thereby encoding relational cues that are essential for generalization.

\paragraph{C2: Calibrated, selective imitation.}
The student should not blindly replicate the teacher’s distribution. 
Instead, it should selectively imitate the teacher’s informative relational structure while suppressing spurious over-confident peaks arising from teacher errors. 
This preserves the benefits of the teacher’s nuanced knowledge without propagating its mistakes.

\subsection{Calibration as a Constraint-based Reformulation}
Motivated by the above requirements, we recast knowledge distillation problem as a teacher calibration problem: we seek a calibration operator $\mathcal{C}$ such that, for each input $x$, the calibrated target $\tilde p_T(\cdot\mid x) = \mathcal{C}\!\big(p_T(\cdot\mid x), x\big)$ is obtained by projecting the raw teacher distribution onto the set of distributions that satisfy the following constraints R1 and R2:
% We formalize the above via a calibration operator $\mathcal{C}$ that maps $p_T$ to a calibrated target $\tilde p_T(\cdot\mid x)=\mathcal{C}\!\big(p_T(\cdot\mid x),x\big)$ subject to explicit reformulated constraints:


\paragraph{R1: Uncertainty with semantic support (for difficulty-aware uncertainty).}
Maintain difficulty-appropriate concentration and guarantee mass over a stable neighborhood of semantically related classes:
\begin{align*}
  h_{\min}(x)\ \le\ H\!\big(\tilde p_T(\cdot\mid x)\big)\ \le\ h_{\max}(x),
  \qquad
  \sum_{k\in\mathcal{N}(y;x)} \tilde p_T(k\mid x)\ \ge\ \alpha(x).
\end{align*}
Here $H(\cdot)$ is an uncertainty measure (e.g., entropy), and $\mathcal{N}(y;x)$ is a semantics-preserving neighborhood of the true label $y$ (e.g., defined via taxonomies, embeddings, or empirical confusion).

\paragraph{R2: Wrong-mass budget (for selective imitation).}

Bound probability assigned to evidently incompatible classes:
\begin{align*}
  \sum_{k\in\mathcal{W}(x,y)} \tilde p_T(k\mid x)\ \le\ \varepsilon(x),
\end{align*}
where $\mathcal{W}(x,y)$ denotes classes known to be inconsistent with $(x,y)$ (e.g., via rules, weak labels, or high-confidence constraints).

\subsection{Projection to Calibrated Targets}
Among all distributions satisfying these constraints, we select the one closest to the original teacher in a structure-preserving sense:
\begin{equation}
\label{eq:proj}
\tilde p_T\ \in\ \arg\min_{q\in\Delta^{C-1}}\ \mathrm{Dist}\!\big(q,\,p_T(\cdot\mid x)\big)
\quad\text{s.t.}\quad \text{R1, R2},
\end{equation}
where $\mathrm{Dist}$ is a structure-sensitive divergence (e.g., symmetrized KL or Wasserstein). Coupled with the training objective in \eqref{eq:student}, this projection emphasizes calibrated pairwise ratios and ordinal relations rather than brittle peak sharpening.
{\color{black}
We prove in Appendix \ref{app:theoretical_analysis} that the optimization problem in \eqref{eq:proj} admits a unique global minimizer without spurious local minima.
}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\textwidth]{iclr2026/figures/main.jpg} 
    \caption{Illustration of the main framework. Left: Difficulty-aware Uncertainty Shaping (DUS) adjusts weights based on the correctness of the model’s predictions, reducing overconfidence and encouraging a more calibrated probability distribution. Right: Wrong-mass Clipping (W-Clip) modifies the probability assigned to incorrect classes when the model makes a wrong prediction, providing a more stable and reliable distribution for the student.
}
    \label{fig:focal_gamma}
\end{figure}





==> iclr2026/sections/03_method.tex <==

\section{Methods}

\subsection{Preliminaries}
\noindent{A. Entropy and Distillation Performance}

Knowledge distillation에서 teacher의 soft output은 student가 학습할 수 있는 중요한 정보를 제공한다. 우리는 먼저 teacher 분포의 entropy와 distillation 성능 간의 상관관계를 분석하였다. 사전 실험 결과, teacher의 출력이 지나치게 날카롭고 확신도가 높은 경우(낮은 entropy), student는 비정답 클래스 간의 관계적 정보를 충분히 전달받지 못해 성능이 저하되었다. 반면, 상대적으로 entropy가 높은 분포는 dark knowledge를 더 풍부하게 담고 있어 distillation 성능을 향상시키는 경향을 보였다. 이는 teacher가 student에게 지식을 전이할 때 있어서 soft distribution 유지의 필요성을 뒷받침한다.


\begin{figure}[h]
    \centering
    \includegraphics[width=0.7\textwidth]{figures/figure1.png} 
    \caption{teacher를 학습할 때, 최종 logits의 top-1 probability에 대한 분포와 entropy값의 분포, 좌측부터 fine tuned teacher, focal loss teacher, focal + entropy teacher(ours)}
    \label{fig:teacher_entropy}
\end{figure}
\begin{table}[h]
    \centering
    \label{tab:teacher_entropy_prob}
    \begin{tabular}{lcc}
        \hline
        \textbf{Teacher} & \textbf{Entropy Avg.} & \textbf{Top-1 Prob Avg.} \\
        \hline
        FT Teacher           & 0.3046 & 0.9400 \\
        Focal Loss  & 0.6586 & 0.8730 \\
        focal + entropy & 2.8188 & 0.4544 \\
        \hline
    \end{tabular}
\end{table}
\begin{table}[h]
    \centering
    \label{tab:banking77}
    \begin{tabular}{lcccc}
        \hline
        \textbf{Banking77} & \textbf{vanilla ft} & \textbf{focal} & \textbf{focal + entropy} \\
        \hline
        student layer 4-256 & ft Teacher & focal ft & focal, entropy \\
        \hline
        teacher      & 93.21 & 93.14 & 91.49 \\
        correct      & 73.53 & 72.88 & 82.14 \\
        wrong        & 68.79 & 72.46 & 77.14 \\
        all          & 73.66 & 72.9 & 82.17 \\
        \hline
    \end{tabular}
    \caption{Banking77 데이터셋에서 서로 다른 Teacher 학습 전략에 따른 성능 비교. 
'vanilla ft'는 일반적인 fine-tuning을 적용한 Teacher, 
'focal'은 Focal Loss만을 적용하여 오답 샘플에 더 집중하도록 학습한 Teacher, 
'focal + entropy'는 Focal Loss에 더해 오답 샘플에 대한
분포의 유연성을 유지하도록 Entropy term을 추가하여 학습한 Teacher를 의미한다.}
\end{table}

\noindent{B. Incorrect Knowledge Transfer}

또 다른 문제는 teacher의 오답이 student에게 직접 전달될 때 발생한다. 사전 실험을 통해 teacher가 잘못된 예측을 강하게 확신하는 경우, student가 이를 그대로 학습하면 오히려 성능이 저하되는 경우가 있다. 이는 기존 KD가 암묵적으로 전제하는 “teacher의 지식은 모두 student에 유용하다”는 가정이 항상 성립하지 않음을 보여준다. 따라서 KD 과정에서 student에 대해서 올바르게 학습하려면 teacher의 오답에 대해 후처리를 하는 것은 반드시 필요한 과정이다.

\subsection{Proposed Methods}

본 연구에서는 위의 분석을 바탕으로, teacher를 distillation 친화적으로 학습시키고, Teacher의 오답이 student에게 해로운 영향을 주지 않도록 제어하는 새로운 방법론을 제안한다. 전체 접근은 두 단계로 구성된다.

\subsubsection{Fine-tuning via Focal Loss}

Teacher 모델 학습 단계에서는, teacher가 오답을 예측하거나 불확실성이 큰 샘플에 대해 집중적으로 학습하도록 하고, 정답을 쉽게 예측하는 경우에는 학습 비중을 낮추는 것을 목표로 한다. 이를 위해 본 연구에서는 focal loss를 활용한다. Focal loss는 본래 class imbalance 문제를 해결하기 위해 제안된 손실 함수로, 각 샘플에 서로 다른 가중치를 부여하여 학습에 반영되는 정도를 조절할 수 있다. 

본 접근법에서는 focal loss를 활용하여, 오답 샘플에 높은 가중치를 부여하고 정답 샘플에는 낮은 가중치를 부여함으로써, teacher가 정답 샘플에 대해 과도하게 확신을 가지는 것을 방지하고, 오답 샘플에 대해서는 학습을 강화하도록 설계하였다. 또한, 오답 샘플에 대해서는 추가적으로 Entropy loss term을 적용하여, teacher의 출력 분포가 단순히 틀린 예측을 나타내는 확률 분포에 그치지 않고, distillation 친화적인 유연한 분포를 갖도록 유도한다. 이를 통해 student가 학습할 때, teacher의 출력 분포가 보다 안정적인 지식을 제공할 수 있다.

Focal loss의 일반적인 정의는 다음과 같다.

\[
\mathcal{L}_{focal} = - \alpha_t (1 - p_t)^\gamma \log(p_t)
\]

여기서 $p_t$는 정답 클래스에 대한 확률, $\alpha_t$는 class weight, $\gamma$은 focusing parameter이다.

추가적으로 오답 샘플에 대해서 Entropy loss를 도입하여, teacher가 오답일 경우에 집중 학습되는 과정에서 과도하게 집중된 분포를 갖지 않도록 조절한다.

오답 샘플 집합 $\mathcal{W}$에 대한 entropy loss는 다음과 같이 정의된다:

\[
\mathcal{L}_{\text{entropy}} = - \frac{1}{|\mathcal{W}|} \sum_{i \in \mathcal{W}} \sum_{c=1}^{C} p_{i,c} \log p_{i,c},
\]

여기서 $p_{i,c}$는 샘플 $i$에 대한 클래스 $c$의 예측 확률이다. 

최종 teacher 학습 손실은 focal loss와 entropy term을 결합하여 다음과 같이 정의된다:

\[
\mathcal{L}_{\text{total}} = \mathcal{L}_{\text{CE}} + \mathcal{L}_{\text{focal}} + \mathcal{L}_{\text{entropy}},
\]



이 과정을 통해 teacher는 정답 클래스에 과도하게 수렴하는 것을 방지하고, 상대적으로 높은 entropy를 유지하는 soft distribution을 출력할 수 있다. Figure~\ref{fig:teacher_entropy}을 통해 확인할 수 있듯이 우리는 이 방식이 teacher의 최종 probability distribution의 entropy를 증가시킴을 확인하였다.

\subsubsection{Post-processing for Wrong Predictions}
두 번째 단계에서는 distillation 과정에서 teacher의 오답이 student에게 직접 전이되지 않도록 probability distribution에 대한 보정(post-processing)을 수행한다. 구체적으로 teacher가 잘못 예측한 경우 해당 클래스의 확률 값을 줄이고 실제 정답 라벨에 재분배한다. 해당 과정 중에 분포의 나머지 부분(dark knowledge)은 유지하도록 하여 오답을 전이하지는 않되, dark knowledge는 student model에 전이할 수 있도록 한다.

teacher의 출력 확률 분포 $\mathbf{p}^{(T)}$가 주어졌을 때, top-1 예측이 실제 레이블과 다를 경우, 잘못된 클래스 k의 확률 $p^{(T)}_k$에서 일부 $\delta$를 정답 레이블 y로 이동시킨다.


\[
\tilde{p}^{(T)}_y = p^{(T)}_y + \delta,
\quad
\tilde{p}^{(T)}_k = p^{(T)}_k - \delta,
\]

여기서 $\delta$는 teacher의 확신 정도(confidence margin)와 entropy를 고려하여 정의된다. 본 연구에서는 다음과 같은 형태를 사용한다.

\[
\delta = \min \Big( \sigma(a \cdot (p^{(T)}_k - p^{(T)}y)) \cdot \big(1 - \tfrac{H}{H{\max}}\big) \cdot (p^{(T)}_k - p^{(T)}_y), \, \eta \cdot p^{(T)}_k \Big)
\]

여기서 H는 teacher 분포의 entropy, $H_{\max} = \log C$ (클래스 개수 C), $\sigma(\cdot)$는 sigmoid 함수, $\eta$는 최대 전이 비율을 제어하는 하이퍼파라미터이다.

이 방식은 teacher의 오답 확신을 억제(confidence suppression)하면서도, 분포에 내재된 dark knowledge는 유지하여 student가 안정적으로 distillation을 받을 수 있도록 한다.

앞서 설명한 두 단계(A: Selective Fine-tuning, B: Post-processing)를 종합하면, 
제안 방법의 전체 학습 절차는 Algorithm~\ref{alg:proposed}와 같다. 
Pseudo code는 teacher의 학습, 오답 보정, 그리고 student distillation의 흐름을 
간결히 나타낸 것이다. 이를 통해 제안 방법이 기존 knowledge distillation과 
어떻게 다른지 한눈에 확인할 수 있다.



==> iclr2026/sections/03_method_en.tex <==
\section{Calibrated Uncertainty Distillation}
While Eq. (2) establishes the theoretical ideal for target calibration, solving this constrained optimization problem directly for every training sample is computationally intractable. 
To bridge this gap, we propose Calibrated Uncertainty Distillation (CUD) designed to \emph{relax} the reformulated constraints (R1, R2) in a practical and modular way.  
Specifically, our practical modules, DUS and W-Clip efficiently approximates the optimal solution: (i) \textbf{DUS}, which reshapes the teacher’s confidence to counter overconfidence while retaining sharp predictions on easy cases, and (ii) \textbf{W-Clip}, which adjusts target distributions to suppress spurious peaks without disturbing relational structure. 
Together, these modules make the constraints operational and yield calibrated soft targets that improve knowledge transfer.



\subsection{Difficult-aware Uncertainty Shaping}
DUS modifies the teacher distribution to provide uncertainty where it is most useful. 
The key idea is to \emph{increase entropy selectively}: ambiguous or misclassified inputs are encouraged to carry higher uncertainty, while confident and correct predictions remain sharp. 
Concretely, we aim to raise entropy only when the teacher is uncertain or wrong—satisfying the lower bound $h_{\min}(x)$—and avoid unnecessary blurring on confident, correct cases to respect the upper bound $h_{\max}(x)$ and maintain class geometry.

Let $p_T(\cdot\mid x)$ be the teacher distribution and $p_T^y \triangleq p_T(y\mid x)$ for ground-truth $y$. We fine-tune the teacher with a \textbf{focal-entropy} objective that down-weights trivial cases and rewards non-degenerate uncertainty on hard or mispredicted inputs:
\begin{equation}
\label{eq:teacher}
\mathcal{L}_{\text{teacher}}
=\lambda_{\mathrm{CE}}\big(-\log p_T^y\big)
+\lambda_{\mathrm{F}}\big(-\alpha_y(1-p_T^y)^{\gamma}\log p_T^y\big)
-\lambda_{\mathrm{H}}\,w(x)\,H\!\big(p_T(\cdot\mid x)\big),
\end{equation}
where $\alpha_y\in(0,1]$, $\gamma\ge 0$, and $H(\cdot)$ denotes entropy. The difficulty gate
\begin{equation*}
w(x)=\mathbbm{1}\{p_T^y<\tau\}+\rho\,(1-p_T^y)^{\beta}
\end{equation*}
activates entropy shaping only when the teacher is wrong or low-confidence. The focal factor $(1-p_T^y)^{\gamma}$ reduces gradients on trivially correct examples ($p_T^y\approx1$) and emphasizes hard/mispredicted ones ($p_T^y$ small); combined with the gated entropy reward $w(x)\,H(\cdot)$, this selectively increases entropy where it improves distillation (meeting $H(\tilde p_T)\!\ge\!h_{\min}(x)$) while leaving easy cases sharp (implicitly respecting $h_{\max}(x)$) without resorting to global label smoothing.


\subsection{W-Clip: Wrong-mass Clipping}
W-Clip calibrates the transfer by reallocating probability mass from clearly wrong classes. 
Instead of reshaping the full distribution, W-Clip applies a budgeted correction that suppresses an overconfident top-1 error when it conflicts with the ground truth. 
Formally, we approximate the wrong-mass constraint $\sum_{k\in\mathcal{W}(x,y)} \tilde p_T(k\mid x)\le \varepsilon(x)$ by suppressing only the wrong top-1 class under a small, controllable budget.

Let $k^\star=\arg\max_k p_T(k\mid x)$ and suppose $k^\star\neq y$. We define two gated amounts
\begin{align}
\label{eq:delta_budget}
\delta_{\mathrm{budget}}(x) &\,\triangleq\, \eta\,p_T(k^\star\mid x),\\
\label{eq:delta_margin}
\delta_{\mathrm{margin}}(x) &\,\triangleq\, m\,\big(p_T(k^\star\mid x)-p_T(y\mid x)\big),
\end{align}
where $\eta\in(0,1)$ caps the total removable mass (the \emph{wrong-mass budget}) and $m\in(0,1]$ scales suppression with the teacher’s over-confidence margin. We then set
\begin{align}
\label{eq:delta_final_b}
\delta(x) &= \min\{\delta_{\mathrm{budget}}(x),\ \delta_{\mathrm{margin}}(x)\},\\
\label{eq:shift_b}
\tilde p_T(y\mid x) &= p_T(y\mid x)+\delta(x),\qquad
\tilde p_T(k^\star\mid x) = p_T(k^\star\mid x)-\delta(x),\\
\tilde p_T(k\mid x) &= p_T(k\mid x)\quad \text{for } k\notin\{y,k^\star\}.
\end{align}
If $k^\star=y$, we simply take $\tilde p_T=p_T$. 

The budget term \eqref{eq:delta_budget} directly implements the constraint that only a limited fraction of wrong-class mass can remain, while the margin term \eqref{eq:delta_margin} focuses corrections on strongly over-confident mistakes. Keeping all non-involved classes unchanged preserves pairwise odds (dark knowledge), so the student inherits informative relations without propagating the teacher’s spurious peak.

\subsection{Student Distillation with Calibrated Targets}
Given the calibrated targets $\tilde p_T(\cdot\mid x)$, the student minimizes a temperatured KL (plus optional CE on labeled data):
\begin{align}
\label{eq:student_kd_b}
\min_{\theta_S}\ \ &\mathbb{E}_{x}\Big[
\lambda_{\mathrm{KD}}\,\tau^2\,\mathrm{KL}\big(\tilde p_T^{(\tau)}(\cdot\mid x)\,\|\,p_S^{(\tau)}(\cdot\mid x;\theta_S)\big)
\Big]\nonumber\\
&\quad +\ \lambda_{\mathrm{CE}}\ \mathbb{E}_{(x,y)}\big[-\log p_S(y\mid x)\big],
\end{align}
where $q^{(\tau)}=\mathrm{softmax}(\log q/\tau)$ and $\tau>0$. This transfers the calibrated structure rather than brittle peaks; unlabeled examples contribute only the KD term, supporting semi-supervised settings.



{\color{black}
\subsection{Operational Realization of Constraints}
\label{subsec:operational_realization}

In Section 2, we formulated target calibration as a constrained projection problem. 
Here, we connect our practical modules to this framework by operationalizing the abstract sets $N(y;x)$ and $W(x,y)$ for the constraints R1 and R2.

\paragraph{Operationalizing Constraint Sets.}
To render the projection tractable, we instantiate these sets based on the principal modes of teacher failure:

\textbf{1. Operational Wrong-Mass Set ($W_{op}$):} We define $W_{op}(x,y) = \{ k^* \}$ strictly when the top-1 prediction $k^*$ contradicts the ground truth ($k^* \neq y$), and $\emptyset$ otherwise. This definition targets the dominant source of semantic misalignment identified in R2.

\textbf{{\color{black}2. Operational Neighborhood Set ($N_{op}$):}} {\color{black}Rather than explicitly defining a semantic neighborhood, we operationalize R1 implicitly. Maximizing entropy via DUS widens the distribution, satisfying the neighborhood mass requirement without pre-defined similarity graph.
}

\paragraph{Approximating the Optimal Projection.}
As proven in Appendix \ref{app:theoretical_analysis}, the optimal solution $q^*$ to the constrained projection is an \textit{exponential tilting} of the teacher distribution. However, computing the partition function for this tilt is computationally expensive.
We demonstrate in Appendix \ref{app:taylor_approx} that \textbf{W-Clip} constitutes a \textit{first-order Taylor approximation} of this exponential tilt around $\nu=0$. Specifically, the linear subtraction in W-Clip recovers the analytical solution ($e^{-\nu} \approx 1-\nu$) for conservative corrections. Similarly, \textbf{DUS} acts as a regularizer that pre-conditions the teacher to satisfy the entropy bounds of R1. Thus, CUD replaces the intractable iterative projection with efficient $O(1)$ arithmetic operations grounded in information geometry.
}

% \paragraph{Design goal.}
% Calibrated Uncertainty Distillation (CUD) is designed to \emph{relax} the reformulated constraints (R1, R2) in a practical and modular way. 
% We introduce two lightweight components: (i) \textbf{DUS}, which reshapes the teacher’s confidence to counter overconfidence while retaining sharp predictions on easy cases, and (ii) \textbf{W-Clip}, which adjusts target distributions to suppress spurious peaks without disturbing relational structure. 
% Together, these modules make the constraints operational and yield calibrated soft targets that improve knowledge transfer.

==> iclr2026/sections/04_experiments_3.tex <==

\subsection{Uncertainy \& OOD Robustness}


% \paragraph{DUS for OOD robustness}
\input{iclr2026/tables/uncertainty}
\input{iclr2026/tables/ece_brier_wrong}

% Claims around calibration and robustness are unsubstantiated. Metrics like ECE or Brier score are absent, and no OOD tests are included.
% Although calibration is claimed to improve OOD robustness, explicit shift experiments (e.g., corrupted or domain-changed data) are missing. 
% OOD 및 ECE 관련 실험 진행

% 우리의 방법론은 intuitive하게

Our approach is explicitly designed to shape predictive uncertainty, so we expect it to provide more reliable confidence estimates and stronger performance on Out-of-Distribution (OOD) detection than standard KD baselines. 
We therefore evaluate both OOD detection and calibration quality.
{\color{black}
\paragraph{OOD Detection}
We follow a standard OOD detection protocol: the teacher and student are trained on Banking77 (in distribution - IND), and we treat CLINC150, MASSIVE, and other intent datasets with different domains and label spaces as OOD. 
We compute AUROC, FPR95, and FPR90 to quantify how well IND and OOD samples are separated.
As shown in Table~\ref{tab:uncertainty}, CUD consistently achieves the highest AUROC and the lowest FPR across all OOD benchmarks. 
The gains are particularly large on heterogeneous OOD datasets such as CLINC150 and MASSIVE, even though the teacher and student never see these domains during training. 
This indicates that the uncertainty shaped by DUS transfers to stronger OOD rejection, not just higher in distribution accuracy.}


{\color{black}
\paragraph{Uncertainty Estimation}
To evaluate how well each model estimates uncertainty, we compute Expected Calibration Error (ECE) and Brier score on the test set of each dataset.
In Table~\ref{tab:ece_wrong}, we report ECE computed only over wrong predictions, where DUS achieves markedly lower values than all KD baselines across every dataset.
This shows that DUS is more capable of signaling its own mistakes, assigning lower confidence when it is wrong, while competing methods remain overconfident even on errors.
Brier scores follow the same trend, confirming that DUS provides more informative uncertainty estimates; detailed results are included in Tab.~\ref{tab:ece} and Fig.~\ref{fig:reliability}.}
We also assess whether confidence separates correct from incorrect predictions by plotting ROC curves on \textsc{Banking77} (in distribution test, label equals correctness). 
As shown in Figure~\ref{fig:auroc-roc}, our method attains a higher AUROC than vanilla KD (0.92 vs.\ 0.83), with a visibly steeper rise in the low FPR region, where selective prediction operates. 
This shows that calibrated targets from CUD produce confidence scores that better rank easy and hard examples, yielding stronger risk coverage trade offs. 
Ablations further reveal that DUS and W Clip individually improve correctness AUROC over vanilla KD (0.90 and 0.88 vs.\ 0.83), while their combination in CUD yields the strongest separation (0.92), suggesting complementary effects. 


==> iclr2026/sections/04_experiments_en.tex <==

\section{Experimental Results}
\label{sec:exp}

\subsection{Training Setup}
\label{subsec:setup}

\paragraph{Models \& Protocol.}
We structure evaluation in two parts. \textbf{(Teacher-side)} We first train a standard \emph{teacher}—\texttt{bert-base-uncased} (12 layers, 768 hidden)—and compare its performance against our distillation-friendly teacher (DUS) under the same data splits. 
\textbf{(Student-side)} We then distill from the trained teacher and compare students across KD methods, using two capacity variants to probe different architectural gaps: \textbf{Mini} (4 layers, 256 hidden), which changes both depth and width so feature-based distillation is inapplicable, and \textbf{Small} (6 layers, 768 hidden), which preserves hidden size and thus admits feature-KD baselines; our method uses calibrated response targets in both cases.  
{\color{black}All results are reported as the mean and variance computed over three independent runs.}

% Origin - 현재 세팅으로 맞춰서 값 일부 수정했습니다.
% \paragraph{Hyperparameters \& Rationale.}
% All runs use AdamW, batch size 32, max length 128, weight decay 0.01, gradient clip 1.0, 10\% linear warmup with cosine decay; the learning rate is selected on a dev split from $\{1\mathrm{e}{-4},\,5\mathrm{e}{-5},\,1\mathrm{e}{-5}\}$ and we report the best dev checkpoint.
% For DUS we set the entropy reward $\lambda_{\mathrm{H}}=0.1$ and focal parameters $\gamma=10.0,\ \alpha_y=1$, which raise uncertainty on hard inputs without global smoothing (supports R1). 
% For W-Clip we use margin $m=10.0$ and wrong-mass budget $\eta=0.5$ to suppress over-confident mistakes while preserving dark knowledge (enforces R2). 
% Student KD uses $\lambda_{\mathrm{KD}}=0.2$, $\lambda_{\mathrm{CE}}=0.8$, and temperature $\tau=1$ to avoid double-softening since targets are already calibrated.

% \paragraph{Hyperparameters \& Rationale.}
% % 하이퍼 파라미터가 꽤나 여러개가 있지만 대부분은 hyperparameter 에 예민하지 않은 값들로 per-dataset performance를 위한 값들 말고 global하게 fixed된 값으로 사용했다. 구체적인 실험 값들을 확인하고 싶으면 appendix참조.
% {\color{black}Our method introduces several hyperparameters, including the entropy reward $\lambda_{\mathrm H}$, focal parameters $\gamma$ and $\alpha_y$, the W-Clip margin $m$ and budget $\eta$, the clipping threshold $W$, and the student distillation weights $\lambda_{\mathrm{KD}}$ and $\lambda_{\mathrm{CE}}$. Rather than performing extensive engineering-style tuning for each dataset, we use a single global configuration across all datasets and architectures rather than performing dataset-specific hyperparameter tuning. All experiments use AdamW with batch size 32, max sequence length 128, weight decay~0.01, gradient clipping at~1.0, and 10\% linear warmup with cosine decay. The only dataset-specific tuning is a small grid search over the learning rate $\{1\mathrm{e}{-4},\, 5\mathrm{e}{-5},\, 1\mathrm{e}{-5}\}$ on a dev split, from which we select the best checkpoint.


% This design is deliberate: our goal is to demonstrate that the proposed method is effective under a single, unified default configuration, without relying on dataset-specific heuristics, fragile parameter choices, or aggressive hyperparameter search. By fixing the distillation-specific hyperparameters across all settings, we emphasize the robustness and general applicability of the method rather than optimizing for per-dataset performance.}


% % The method introduces many hyperparameters, but only γ is tuned. The rest are fixed without justification, which weakens the claim of being architecture-agnostic. .Why clip at W=3.0 for example weighting? This seems arbitrary.

% {\color{black}
% The example weighting mechanism employs a clipped weight,
% \[
% w_{\text{clip}}(x) = \min(W,\, w_{\text{raw}}(x)),
% \]
% where $W$ acts as an upper bound on per-example weights. This clipping prevents a small number of outlier or extremely hard examples from dominating the learning signal, which can destabilize training, while still allowing genuinely difficult examples to receive larger weights than easy ones.

% A natural question is whether the choice of $W = 3.0$ is arbitrary. In practice, the presence of clipping itself is more important than the precise value of $W$. Empirically, varying $W \in \{3,4,5\}$ yields nearly identical performance across all models and datasets, with no consistent trend suggesting that any value is preferable. This indicates that the method is inherently robust to the choice of $W$ within a reasonable range.

% Given this insensitivity, we set $W = 3.0$ as a conservative and architecture-agnostic ``safety cap’’ that (i) limits the influence of extreme examples, (ii) avoids unnecessary hyperparameter tuning, and (iii) remains stable across datasets and architectures. Thus, $W$ is best interpreted as a stability-oriented regularization constant, rather than a finely tuned performance-critical hyperparameter. Unless stated otherwise, all reported results use this shared default setting.
% }

\paragraph{Hyperparameters \& Rationale.}
{\color{black}
While our method introduces several hyperparameters, most show low sensitivity; we tuned them once on the Banking dataset and used the same global values for all tasks, avoiding per-dataset hyperparameter engineering (see Appendix \ref{app:parameters}).
The key distillation parameters include the entropy reward $\lambda_{\mathrm H}=0.1$, the focal parameters $\gamma=10$ and $\alpha_y=1$, and the entropy based gating $m = 0.7$ and weighting $\eta = 0.5$, and together these values behave such that smaller settings recover a standard distillation baseline while larger settings amplify the inductive bias of our approach. 
In addition, several minor scalar ratios $\lambda_{\mathrm{KD}}$ and $\lambda_{\mathrm{CE}}$.
All experiments use AdamW with batch size 32, maximum sequence length 128, weight decay $0.01$, gradient clipping at $1.0$, and $10\%$ linear warmup with cosine decay.
}





% \paragraph{Benchmarks \& Evaluation.}
% To test distillation under \emph{single-label} multiclass settings with diverse cardinalities, we evaluate on seven text-classification datasets spanning 2–150 classes: \textbf{Banking77} (77 intents; banking customer-support intents)~\citep{larson2019banking77}, \textbf{CLINC150} (150 intents; open-domain intents, in-scope)~\citep{casanueva2020dual}, \textbf{MASSIVE} (60 intents; multilingual SLU intents, English subset unless noted)~\citep{fitzgerald2022massive}, \textbf{TREC} (6 question types; coarse question classification)~\citep{taware2021text}, and \textbf{AG~News} (4 topics; news topic classification). For broader NLU coverage we additionally report GLUE tasks in the appendix—\textbf{MNLI} (3-way NLI)~\citep{williams2018mnli}, \textbf{SST-2} (binary sentiment)~\citep{socher2013sentiment}, \textbf{QNLI} (binary NLI derived from SQuAD)~\citep{rajpurkar2016squad}, and \textbf{QQP} (binary duplicate-question detection)~\citep{chen2018quora}. Following prior work~\citep{park2021student,hu2022survey}, we report \emph{accuracy} on the test splits.

% 벤치마크에 대한 수정
\paragraph{Benchmarks \& Evaluation.}
We evaluate our method on five classification datasets spanning a wide range of label granularities, from 4 to 150 classes: Banking77 (77 intents) \citep{larson2019banking77}, CLINC150 (150 intents) \citep{casanueva2020dual}, MASSIVE (60 intents) \citep{fitzgerald2022massive}, TREC (6 question types) \citep{li2002learning}, and AG News (4 topic categories) \citep{zhang2015character}. Detailed dataset statistics are provided in Table~\ref{tab:benchmark} of the Appendix~\ref{app:benchmarks}. Additional results on binary classification settings are also included in the Appendix for completeness.


\paragraph{Baselines.}
We compare against representative KD methods, summarized by their characteristics:
\begin{enumerate}
\item \textbf{LKD (Logit-KD)}~\citep{hinton2015distilling}: Response-based KL matching on teacher soft logits (with temperature). Simple and task-agnostic but ignores intermediate structure.

\item \textbf{PKD (Patient KD)}~\citep{sun2019patient}: Layer-wise alignment of hidden representations. \emph{Exploits intermediate features and depth supervision}; effective when student width/layers can be mapped to the teacher, less suited to severe architectural mismatch. 

\item \textbf{TinyBERT}~\citep{jiao2020tinybert}: Distills both self-attention and hidden states, originally with two-stage training and data augmentation. \emph{Achieves high compression quality via rich feature-level objectives}; in our setup, we disable augmentation for a fair task-specific comparison.

{\color{black}
\item \textbf{CKD (Contextual KD)}~\citep{park2021ckd}: Transfers \emph{relational knowledge} by modeling two forms of contextual structure: \emph{Word Relation} between tokens, and \emph{Layer Transforming Relation} across layers. Architecture-agnostic and effective for heterogeneous teacher–student pairs.

\item \textbf{MGSKD (Multi-Granularity Structural KD)}~\citep{liu2021mgskd}: Distills \emph{structural relations} over \emph{multiple semantic granularities} (tokens, spans, samples), formulated via pair-wise interactions and triplet geometric angles. Preserves richer linguistic structure than mono-granularity KD, at the cost of higher relational computation.
}

\item \textbf{AD-KD}~\citep{wu2023ad}: Response-based distillation with confidence/uncertainty-aware reweighting or calibration. \emph{Mitigates propagation of over-confident teacher errors} while keeping architecture independence and low overhead.
\end{enumerate}

\input{iclr2026/tables/main_old}


% \subsection{Main Results}
% \label{subsec:results}
% Table~\ref{tab:kd_results} compares (i) \emph{teacher-side} performance after standard fine-tuning versus our distillation-friendly teacher, and (ii) \emph{student-side} performance after distillation across two capacity regimes. The trends are consistent with our design: the benefit of calibrated distillation grows with the number of classes (richer dark knowledge), while it diminishes—and can even turn neutral—on binary tasks where the teacher’s distribution reduces to $(p,1-p)$ and R1/R2 collapse toward ordinary temperature scaling or label smoothing.

% \textbf{Small student (6L–768D).} With a width-matched student, all methods are near the teacher’s ceiling (avg 94.32). Our calibrated KD (CUD) gives a modest but consistent lift over Vanilla KD (avg $+0.38$ points; 93.07 vs.\ 92.69), surpassing or matching alternatives on most datasets (e.g., TREC $97.4$ vs.\ teacher $97.0$). The small deltas reflect limited headroom: when the student has sufficient capacity and feature geometry is preserved, intermediate-feature baselines (PKD/TinyBERT) are competitive and response calibration yields incremental gains.

% \textbf{Mini student (4L–256D).} When both depth and width shrink, representation matching is infeasible and response targets dominate. Here CUD shows clear advantages on high-cardinality tasks: Banking77 ($+11.1$ over Vanilla), MASSIVE ($+5.8$), CLINC150 ($+7.1$), though AD-KD is the strongest on this dataset), driving the best average among response-based methods (88.73 vs.\ 85.14 for Vanilla). These are precisely the settings where preserving teacher uncertainty over \emph{many} plausible alternatives helps the student recover fine-grained class relations. On low-cardinality tasks the picture tightens: AGNews (4-way) is near-saturated and our wrong-peak suppression can slightly perturb an already sharp yet correct distribution ($-0.39$ vs.\ Vanilla).

% \textbf{Why multiclass helps (and binary often does not).} For large $C$, R1 raises entropy on hard inputs while R2 caps mass on the specific wrong peak, preserving the \emph{relative} odds over the remaining $(C{-}2)$ classes. This retains informative neighborhoods that the student can imitate, improving sample efficiency and robustness. In contrast, with $C{\in}\{2,3\}$ the teacher’s uncertainty structure is nearly one-dimensional; suppressing a wrong peak is almost equivalent to re-tempering logits, so our calibrated shift provides little extra signal and may slightly interfere when the teacher is already well-calibrated. Practically, the method is most impactful for intent/topic taxonomies with tens to hundreds of classes (e.g., Banking77/CLINC/MASSIVE) and yields smaller gains when $C\!\ge\!4$ or when the student nearly matches the teacher in capacity.

% \textbf{Other Observations.} (a) On CLINC150 (Mini), AD-KD attains the top score, suggesting that more aggressive confidence-aware reweighting can be beneficial on that distribution; our projection is conservative by design to preserve dark knowledge, and the two approaches may be complementary. (b) On TREC (6-way), even small students approach or exceed the teacher, indicating that calibrated targets help most where teacher errors are concentrated on a few confusable classes. (c) Across both capacities, the average gaps shrink as architectural mismatch decreases, reinforcing that response calibration particularly matters when feature alignment is hard. 
% Calibrated uncertainty distillation is most effective \emph{as class cardinality and ambiguity increase} and \emph{as the teacher–student gap widens}.




\subsection{Main results}
\label{subsec:results}

Table~\ref{tab:kd_results} reports both teacher side and student side performance. 
Across all datasets and student capacities, CUD consistently outperforms prior baselines. 

\textbf{Effect of student capacity.}
For the larger student (6L 768D), several baselines already achieve accuracy comparable to the teacher (teacher average 94.32). 
In this regime CUD still attains the best average student performance (94.33), improving over vanilla logit KD by about {$+1.0$} point on average (94.33 versus 93.33). 
For the smaller student (4L 256D), the dimensionality gap to the teacher makes representation–level matching difficult or even infeasible, so performance is largely determined by the quality of the response targets. 
In this regime, CUD delivers substantially clearly outperforming other baselines with larger margin. 

\textbf{Effect of the cardinality.}
CUD yields much larger gains, especially on tasks with many classes such as Banking77, CLINC150, MASSIVE, where it improves over vanilla KD by $+10.43$, $+5.14$, and $+5.22$ points respectively. 
This pattern matches our intuition: on tasks with many classes, the calibrated targets keep meaningful probability on several plausible labels while suppressing the dominant wrong peak, so the student can imitate a richer set of alternatives. 
In contrast, when the number of classes is small, for example (AGNews, TREC), the teacher distribution is already almost deterministic and offers little additional structure to recover.
For extremely small numbers of classes (binary), this effect becomes stronger; suppressing a wrong peak acts like mild logit re-tempering and adds little information beyond standard smoothing or temperature scaling. Detailed analysis are provided in the Appendix \ref{app:binary}.





==> iclr2026/sections/05_analysis.tex <==

% \section{Analysis}





% \color{red}
% \subsection{Comparison with Temperature Scaling \& Label Smoothing}

% \color{black}




==> iclr2026/sections/05_analysis_en.tex <==


\section{Analysis}

\subsection{Ablation Study}

\input{iclr2026/tables/ablation}
{\color{black}
Table~\ref{tab:ablation} reports ablations of our main modules (DUS and W-Clip) in the 4L–256D student.
While both components improve over vanilla KD on average, and the gains grow with label cardinality as noted in the main results, the detailed breakdown further reveals when and why they matter.
}

\paragraph{Closing the teacher–student gap.}
Relative to the fine-tuned teacher, vanilla KD leaves substantial headroom: $-13.09$ points on Banking77 (80.61 vs.\ 93.70), $-8.0$ on CLINC150 (88.35 vs.\ 96.35), and $-7.43$ on MASSIVE (82.04 vs.\ 89.47).CUD closes 80\%, 63\%, and 75\% of these gaps respectively, demonstrating that calibrated uncertainty specifically helps students recover performance where naive KD collapses.

\paragraph{Relative impact of modules.}
DUS alone outperforms W-Clip in average accuracy (92.24 vs.\ 91.66), showing that reshaping the teacher distribution is more fundamental than just reweighting samples. W-Clip is beneficial in high-class regimes (e.g., $+8.64$ on Banking77 and $+4.33$ on MASSIVE vs.\ vanilla KD), but can over-emphasize noise in easier tasks. The full CUD system balances both: projection (R2) prevents over-amplification of wrong peaks while clipped weighting emphasizes informative errors, producing the most stable and highest average (92.49, $\Delta{+}4.27$).

\paragraph{Teacher calibration.}
In our setup, DUS trained teacher attains slightly lower accuracy than a standard fine tuned teacher (Tab.~\ref{tab:ft_cud}), yet students distilled from it consistently outperform those distilled from the standard teacher. 
This holds not only for our CUD objective but also for other KD baselines when we simply replace their original teacher with ours (teacher side ablations in Tab.~\ref{tab:apply_our_teacher}). 



% \subsection{Can CUD better separate correct from incorrect predictions?}

% We assess whether a model’s confidence separates correct from incorrect predictions by plotting ROC curves on \textsc{Banking77} (ID test; label = correctness). 
% As shown in Fig.~\ref{fig:auroc-roc}, CUD attains a higher AUROC than Vanilla KD (0.92 vs.\ 0.83), with a visibly steeper rise in the low-FPR region—precisely where selective prediction operates. 
% This threshold-free improvement indicates that calibrated targets from CUD produce confidence scores that better rank easy vs.\ hard examples, yielding stronger risk–coverage trade-offs.
% {\color{black}
% Decomposing the effect shows that both DUS and W-Clip individually improve correctness AUROC over Vanilla KD (0.83), achieving 0.90 and 0.88 respectively. This indicates that each component contributes meaningfully on its own by refining the teacher’s uncertainty structure and emphasizing informative examples. However, combining the two in CUD yields the strongest improvement (0.92), as their complementary behaviors reinforce each other. In other words, the joint use of DUS and W-Clip provides the most effective separation between correct and incorrect predictions, resulting in the highest correctness AUROC.
% }
% Despite the DUS teacher’s slightly lower standalone accuracy in our setup, CUD’s higher correctness AUROC shows that \emph{how well confidence ranks errors} matters more for student utility than the teacher’s peak accuracy.

\input{iclr2026/tables/auroc}

\subsection{The Role of \texorpdfstring{$\gamma$}{gamma}: Balancing accuracy and Calibrated uncertainty}
We study how $\gamma$ in DUS reshapes the teacher distribution and student performance. 
Since the per-example weight scales as $(1-p_T^y)^{\gamma}$, increasing $\gamma$ aggressively down-weights correct examples and emphasizes wrong ones. 
Empirically (Fig.~\ref{fig:auroc-gamma}), larger $\gamma$ produces a \emph{softer} top-1 distribution: the sharp peak near $\approx\!0.95$ collapses while probability mass shifts toward mid confidence (0.5–0.9). 
Thus, there is a clear \textbf{inverse relation} between $\gamma$ and top-1 concentration/peak height (and, equivalently, a positive relation with entropy on hard cases).
This softening is beneficial for transfer up to a point. 
On the dev sweep shown, student accuracy rises monotonically as $\gamma$ increases from $3$ to $10$ (0.85$\rightarrow$0.89); table at right), indicating that \emph{within this range} recovering teacher uncertainty improves the ranking signal distilled to the student. 
% However, very large $\gamma$ can over-flatten easy cases and erode class geometry; in practice we select a \emph{moderate} $\gamma$ that achieves sufficient softening without globally blurring the distribution. 
In our experiments, the $\gamma$ sweep further illustrates the transfer-first trade-off: modest increases in teacher uncertainty (sometimes with a minor drop in the teacher’s standalone accuracy) correlate with \emph{higher} student accuracy after KD, reinforcing that calibrating the teacher for \emph{distillability} can be preferable to maximizing its peak accuracy.




==> iclr2026/sections/06_related.tex <==
\section{Related Work}

Knowledge distillation (KD) fundamentally relies on transferring the "knowledge" encoded in soft targets~\citep{hinton2015distilling}, yet standard teachers often exhibit overconfidence that degrades this signal. While calibration techniques~\citep{guo2017calibration} and regularizers like label smoothing~\citep{muller2019does} or confidence penalties~\citep{pereyra2017regularizing} address predictive sharpness, they risk indiscriminately blurring the fine-grained inter-class geometry essential for effective transfer. Furthermore, prior attempts to optimize teachers for distillation~\citep{menon2021statistical,dong2024student} or align intermediate features~\citep{sun2019patient} often lack difficulty-awareness or impose strict architectural constraints. In contrast, our approach targets the \emph{distributional shape} of the transfer; we jointly optimize the teacher to maintain difficulty-aware uncertainty through selective entropy shaping (DUS) and apply a constrained projection (W-Clip) to suppress specific wrong-class peaks without distorting the informative pairwise relations among background classes. 
For an extended review of related literature, please refer to the Appendix \ref{app:extedrelatedwork}.


==> iclr2026/sections/07_conclusion.tex <==
\section{Conclusion}
We presented \emph{Calibrated Uncertainty Distillation (CUD)}, a simple architecture-agnostic dual distillation mechanism. 
Unlike conventional approaches that treat the teacher as fixed, CUD explicitly reshapes the teacher to retain difficulty-aware uncertainty and calibrates the transfer to suppress over-confident mistakes while preserving informative class relations. 
Empirically, CUD delivers consistent surpass stronger other baselines, highlighting the value of calibrated distributions over sharpened certainty. 
% These results show that effective distillation depends not only on \emph{how} knowledge is transferred but also on \emph{what} distributional structure the teacher provides. 

\clearpage

\section*{Limitations}
Our work has several limitations. {\color{black}First, we restrict evaluation to single-label classification, leaving open the extension to multi-label, sequence-level, or generative tasks where calibration constraints may require new formulations.} Second, our projection rules rely on fixed hyperparameters (e.g., entropy weights, wrong-mass budget), which, while effective, may not optimally adapt across domains or dynamic training conditions. 
% Third, we focus on response-based transfer only and do not combine with feature-level or relation-based KD, which could provide complementary benefits when teacher and student architectures are aligned. 
Third, the benefits of calibrated uncertainty are reduced on binary or very small-class problems, where the teacher’s uncertainty structure becomes nearly one-dimensional; in such cases, suppressing a wrong peak is almost equivalent to mild logit re-tempering, providing limited additional signal beyond classical smoothing or temperature scaling. Finally, our experiments are conducted on standard benchmarks; validation under real-world distribution shift, selective prediction, and resource-limited scenarios is an important next step.
{\color{black}These limitations suggest several directions for future work: adaptive per-example calibration, integration with semantic neighborhoods or taxonomies, and applications beyond classification toward generative modeling.}
We believe exploring these avenues will further enhance the role of calibrated uncertainty in distillation and broaden the impact of compact, trustworthy models in practice.

==> iclr2026/tables/ablation.tex <==
% \begin{table}[t]
% \centering
% \small
% \setlength{\tabcolsep}{14pt}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{lccccc}
% \toprule
% \textbf{Dataset (Classes)} & \textbf{FT teacher} & \textbf{vanilla KD} & \textbf{W-Clip} & \textbf{DUS} & \textbf{CUD} \\
% \midrule
% Banking77 (77)   & 93.21 & 78.83 & 79.41 & 83.34 & 84.80 \\
% Clinc150 (150)   & 96.35 & 80.28 & 84.40 & 86.13 & 87.33 \\
% TREC (6)         & 97.00 & 95.80 & 95.40 & 96.40 & 96.20 \\
% AGNews (4)       & 94.56 & 94.39 & 94.23 & 94.14 & 94.00 \\
% Massive (60)     & 89.47 & 81.45 & 86.71 & 87.11 & 87.21 \\
% QNLI (2)         & 90.66 & 83.56 & 82.62 & 84.14 & 84.09 \\
% SST-2 (2)        & 90.82 & 86.81 & 86.23 & 87.27 & 87.50 \\
% \midrule
% \textbf{Average}            & 93.15 & 85.87 & 84.69 & 85.59 & 88.73 \\
% \bottomrule
% \end{tabular}}
% \caption{Results of different distillation strategies on multiple datasets (class counts indicated) with the 4-layer, 256-hidden student model. Our method (CUD) achieves the best average performance.}
% \label{tab:kd_results_4layer_transposed_final}
% \end{table}


% \begin{table}[t]
% \centering
% \small
% \setlength{\tabcolsep}{4pt}
% \begin{tabular}{lcccccccc}
% \toprule
%  & \textbf{Banking77} & \textbf{Clinc150 } & \textbf{TREC} & \textbf{AGNews} & \textbf{Massive} & \textbf{QNLI} & \textbf{SST-2} & \textbf{Avg} \\
% \midrule
% FT teacher    & 93.21 & 96.35 & 97.00 & 94.56 & 89.47 & 90.66 & 90.82 & 93.15 \\
% vanilla KD    & 78.83 & 80.28 & 95.80 & 94.39 & 81.45 & 83.56 & 86.81 & 85.87 \\
% W-Clip        & 79.41 & 84.40 & 95.40 & 94.23 & 86.71 & 82.62 & 86.23 & 84.69 \\
% DUS           & 83.34 & 86.13 & 96.40 & 94.14 & 87.11 & 84.14 & 87.27 & 85.59 \\
% CUD(ours)     & 84.80 & 87.33 & 96.20 & 94.00 & 87.21 & 84.09 & 87.50 & 88.73 \\
% \bottomrule
% \end{tabular}
% \caption{Results of different distillation strategies on multiple datasets with the 4-layer, 256-hidden student model. Our method (focal+process) achieves the best average performance.}
% \label{tab:kd_results_4layer}
% \end{table}

% % Requires: \usepackage{booktabs}
% \begin{table}[t]
% \centering
% \small
% \setlength{\tabcolsep}{4pt}
% \caption{Teacher reference vs.\ student distillation variants (4-layer, 256-hidden student). 
% \textbf{DUS} = Distillation Uncertainty Shaping (R1; focal–entropy teacher, no post-hoc projection). 
% \textbf{W-Clip} = clipped example reweighting. 
% \textbf{CUD} = DUS + wrong-peak projection (R2) + W-Clip. 
% Averages are across all datasets; the rightmost column shows the average gain over Vanilla KD.}
% \label{tab:kd_results_4layer}
% \begin{tabular}{lcccccccc c}
% \toprule
% \textbf{Configuration} & \textbf{Banking77} & \textbf{CLINC150} & \textbf{TREC} & \textbf{AGNews} & \textbf{MASSIVE} & \textbf{QNLI} & \textbf{SST-2} & \textbf{Avg} & \textbf{Avg $\Delta$ vs KD} \\
% \midrule
% \multicolumn{10}{l}{\textit{Teacher (reference, bert-base-uncased; not directly comparable to student capacity)}} \\
% FT Teacher 
% & 93.21 & 96.35 & 97.00 & 94.56 & 89.47 & 90.66 & 90.82 & 93.15 & --- \\
% \midrule
% \multicolumn{10}{l}{\textit{Student (4L–256D) with different distillation variants}} \\
% Vanilla KD 
% & 73.66 & 80.28 & 95.80 & 94.39 & 81.45 & 83.56 & 86.81 & 85.14 & \phantom{+}0.00 \\
% KD + DUS (R1 only) 
% & 83.34 & 86.13 & 96.40 & 94.14 & 87.11 & 84.14 & 87.27 & 85.59 & \phantom{+}0.45 \\
% KD + W-Clip 
% & 79.41 & 84.40 & 95.40 & 94.23 & 86.71 & 82.62 & 86.23 & 84.69 & $-0.45$ \\
% \textbf{KD + DUS + W-Clip (CUD)} 
% & \textbf{84.80} & \textbf{87.33} & \textbf{96.20} & \textbf{94.00} & \textbf{87.21} & \textbf{84.09} & \textbf{87.50} & \textbf{88.73} & \textbf{+3.59} \\
% \bottomrule
% \end{tabular}
% \end{table}

% % Requires: \usepackage{booktabs}
% \begin{table}[t]
% \centering
% \small
% \setlength{\tabcolsep}{4pt}
% \begin{tabular}{lcccccccc c}
% \toprule
% \textbf{Method (4L–256D student unless noted)} & \textbf{Banking77} & \textbf{CLINC150} & \textbf{TREC} & \textbf{AGNews} & \textbf{MASSIVE} & \textbf{QNLI} & \textbf{SST-2} & \textbf{Avg} & \boldmath$\Delta$ \textbf{vs KD} \\
% \midrule
% \emph{Teacher (FT, no KD)}                     & 93.21 & 96.35 & 97.00 & 94.56 & 89.47 & 90.66 & 90.82 & \textbf{93.15} & -- \\
% \midrule
% KD (baseline)                                   & 78.83 & 80.28 & 95.80 & 94.39 & 81.45 & 83.56 & 86.81 & \textbf{85.87} & \phantom{+}0.00 \\
% KD + DUS (R1 teacher only)                      & 83.34 & 86.13 & 96.40 & 94.14 & 87.11 & 84.14 & 87.27 & \textbf{88.36} & +3.22 \\
% KD + W-Clip                                     & 79.41 & 84.40 & 95.40 & 94.23 & 86.71 & 82.62 & 86.23 & \textbf{87.00} & +1.86 \\
% KD + DUS + W-Clip (\textbf{CUD}, ours)          & 84.80 & 87.33 & 96.20 & 94.00 & 87.21 & 84.09 & 87.50 & \textbf{88.73} & \textbf{+3.59} \\
% \bottomrule
% \end{tabular}
% \caption{Teacher accuracy (top) and student accuracy after distillation (bottom) on seven datasets.
% \emph{KD} is vanilla response-based distillation; \emph{DUS} applies our R1 distillation-friendly teacher without projection; \emph{W-Clip} clips example reweighting; \emph{CUD} combines R1 + W-Clip (full method). Avg is the mean across tasks; $\Delta$ vs KD reports average gain over the KD baseline.}
% \label{tab:kd_results_4layer_clean}
% \end{table}

% Requires: \usepackage{booktabs}
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\resizebox{\textwidth}{!}{
{\color{black}
\begin{tabular}{lccccc cc}
\toprule
\textbf{Configuration} & \textbf{Banking77} & \textbf{CLINC150} & \textbf{TREC} & \textbf{AGNews} & \textbf{MASSIVE} & \textbf{Avg} & \textbf{AVG $\Delta$} \\
\midrule
\textbf{Teacher} (\emph{FT, no KD})
& 93.70 & 96.35 & 97.40 & 94.69 & 89.47 & 94.32 & --- \\
\midrule
\multicolumn{8}{l}{\textit{Student (4L–256D) with distillation variants}} \\
LKD
& 80.61 & 88.35 & 95.80 & \textbf{94.31} & 82.04 & 88.22 & \phantom{+0.00} \\
LKD + DUS
& 90.62 & 93.24 & 96.40 & 94.17 & 86.76 & 92.24 & +4.02 \\
LKD + W-Clip 
& 89.25 & 93.02 & 95.40 & 94.28 & 86.37 & 91.66 & +3.44 \\
\midrule
\textbf{CUD (Ours) } 
& \textbf{91.22} & \textbf{93.45} & \textbf{96.47} & 94.11 & \textbf{87.22} & \textbf{92.49} & \textbf{+4.27} \\
\bottomrule
\end{tabular}
}
}
\caption{{\color{black}\textbf{Ablation of our model on multiclass benchmarks.}
We evaluate the individual contributions of DUS and W-Clip in a 4-layer, 256-dim student. Both modules provide measurable improvements over LKD, and their combination in CUD delivers the strongest gains.}}
\label{tab:ablation}
\end{table}

==> iclr2026/tables/apply_our_teacher.tex <==
% \begin{table}[h!]
% \centering
% \setlength{\tabcolsep}{10pt}
% \resizebox{\textwidth}{!}{
% {\color{black}
% \begin{tabular}{llccccc}
% \toprule
% \textbf{Baseline} & \textbf{Method} & \textbf{Banking77} & \textbf{Clinc150} & \textbf{TREC} & \textbf{AGNews} & \textbf{Massive} \\
% \midrule
% \multirow {TinyBERT} 
%     & ft teacher      & 89.74 & 88.44 & 93.4 & 94.31 & 89.12 \\
%     & ours            & \textbf{91.29} & \textbf{92.91} & \textbf{96.8} & \textbf{94.36} & \textbf{89.27}  \\
% \midrule
% \multirow {MGSKD} 
%     & ft teacher      & 91.65 & 95.62 & 97 & \textbf{94.81} & 88.88 \\
%     & ours            & \textbf{91.92} & \textbf{95.91} & \textbf{97.2} & 94.44 & \textbf{89.27} \\
% \midrule
% \multirow {CKD} 
%     & ft teacher      & 93.76 & 96.11 & 97.8 & \textbf{94.89} & 89.57 \\
%     & ours            & \textbf{93.86} & \textbf{97.03} & 97.8 & 94.73 & \textbf{89.86} \\
% \midrule
% \multirow {ADKD} 
%     & ft teacher      & 93.05 & 95.53 & 96.4 & \textbf{94.82} & \textbf{89.62} \\
%     & ours            & \textbf{93.08} & \textbf{95.77} & \textbf{97.6} & 94.55 & 89.32 \\
% \bottomrule
% \end{tabular}}}
% \caption{{\color{black}Comparison of layer-6 student performance when using a conventionally fine-tuned teacher (ft teacher) versus our CUD-trained teacher (ours) as the distillation source.}}
% \label{tab:apply_our_teacher}
% \end{table}
\begin{table}[h!]
\centering
\small
\begingroup % 전체 표를 파랗게
\setlength{\tabcolsep}{12pt}

\resizebox{\textwidth}{!}{
{\color{black}
\begin{tabular}{llccccc}
\toprule
\textbf{Baseline} & \textbf{Method} & \textbf{Banking77} & \textbf{Clinc150} & \textbf{TREC} & \textbf{AGNews} & \textbf{Massive} \\
\midrule

\multirow{2}{*}{TinyBERT} 
    & ft teacher      & 89.74 & 88.44 & 96.20 & 94.31 & 89.12 \\
    & ours            & \textbf{91.29} & \textbf{92.91} & \textbf{96.80} & \textbf{94.36} & \textbf{89.27} \\
\midrule

\multirow{2}{*}{MGSKD} 
    & ft teacher      & 91.62 & 95.46 & 87.80 & \textbf{94.81} & 88.88 \\
    & ours            & \textbf{91.92} & \textbf{95.91} & \textbf{97.20} & 94.44 & \textbf{89.27} \\
\midrule

\multirow{2}{*}{CKD} 
    & ft teacher      & 93.76 & 96.11 & 97.80 & \textbf{94.89} & 89.57 \\
    & ours            & \textbf{93.86} & \textbf{97.03} & 97.80 & 94.73 & \textbf{89.86} \\
\midrule

\multirow{2}{*}{AD-KD} 
    & ft teacher      & 93.05 & 95.53 & 96.40 & \textbf{94.82} & \textbf{89.62} \\
    & ours            & \textbf{93.08} & \textbf{95.77} & \textbf{97.60} & 94.55 & 89.32 \\
\bottomrule
\end{tabular}
}
}
\caption{{\color{black}Comparison of layer-6 student performance using a fine-tuned teacher vs.\ our CUD-trained teacher.}}
\label{tab:apply_our_teacher}

\endgroup
\end{table}

==> iclr2026/tables/auroc.tex <==
\begin{figure*}[t]
    \begin{subfigure}{.5\linewidth}
        \centering
        \includegraphics[width=0.99\linewidth]{iclr2026/figures/roc_modules_resize.png}
        \caption{ROC curves comparing confidence-based correctness separation. }
        \label{fig:auroc-roc}
    \end{subfigure}
    \begin{subfigure}{.5\linewidth}
        \centering
        \includegraphics[width=0.99\linewidth]{iclr2026/figures/figure_gamma_resize.png}
        \caption{Teacher probability distributions under varying $\gamma$. Higher $\gamma$ values soften over-confident peaks.}
        \label{fig:auroc-gamma}
    \end{subfigure}
    \caption{Effect of calibration on uncertainty and distributions.}
    
    \label{fig:auroc}
\end{figure*}

==> iclr2026/tables/benchmark.tex <==
% \begin{table}[h!]
% \centering
% \small
% \setlength{\tabcolsep}{8pt}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{lccc p{5.2cm}}
% \toprule
% \textbf{Dataset} & \textbf{\#Classes} & \textbf{Domain} & \textbf{Task Type} & \textbf{Description} \\
% \midrule
% \textbf{Banking77} & 77 & Customer Support & Intent Classification & A fine-grained intent dataset for banking-related customer queries ~\citep{larson2019banking77}. \\
% \midrule
% \textbf{CLINC150} & 150 & Open-domain & Intent Classification & Wide-coverage natural language intent dataset with 150 classes across multiple domains~\citep{casanueva2020dual}. \\
% \midrule
% \textbf{MASSIVE} & 60 & Multilingual SLU & Intent Classification & Multilingual dataset for SLU tasks; English subset used unless otherwise stated~\citep{fitzgerald2022massive}. \\
% \midrule
% \textbf{TREC} & 6 & Question Answering & Question Type Classification & Coarse-grained question type labels for factoid QA tasks ~\citep{li2002learning}. \\
% \midrule
% \textbf{AG News} & 4 & News & Topic Classification & News article classification into 4 broad topical categories ~\citep{zhang2015character}. \\
% \bottomrule
% \end{tabular}
% }
% \caption{Metadata summary of the benchmark datasets used in our evaluation.}
% \label{tab:benchmark}
% \end{table}


\begin{table}[h!]
\centering
\setlength{\tabcolsep}{8pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{
    >{\centering\arraybackslash}m{2.3cm}  % Dataset
    >{\centering\arraybackslash}m{1.8cm}  % #Classes
    >{\centering\arraybackslash}m{2.5cm}  % Domain
    >{\centering\arraybackslash}m{3cm}    % Task Type
    >{\centering\arraybackslash}m{7.5cm}  % Description
}
\toprule
\textbf{Dataset} & \textbf{\#Classes} & \textbf{Domain} & \textbf{Task Type} & \textbf{Description} \\
\midrule
\textbf{Banking77} & 77 & Customer Support & Intent Classification & 
A fine-grained intent dataset for banking-related customer queries 

~\citep{larson2019banking77}. \\
\midrule
\textbf{CLINC150} & 150 & Open-domain & Intent Classification &
Wide-coverage natural language intent dataset with 150 classes across multiple domains 

~\citep{casanueva2020dual}. \\
\midrule
\textbf{MASSIVE} & 60 & Multilingual SLU & Intent Classification &
Multilingual dataset for SLU tasks; English subset used unless otherwise stated 

~\citep{fitzgerald2022massive}. \\
\midrule
\textbf{TREC} & 6 & Question Answering & Question Type Classification &
Coarse-grained question type labels for factoid QA tasks ~\citep{li2002learning}. \\
\midrule
\textbf{AG News} & 4 & News & Topic Classification &
News article classification into 4 broad topical categories ~\citep{zhang2015character}. \\
\bottomrule
\end{tabular}}
\caption{Metadata summary of the benchmark datasets used in our evaluation..}
\label{tab:benchmark}
\end{table}



==> iclr2026/tables/binary.tex <==
\begin{table*}[ht]
\centering
\small
\setlength{\tabcolsep}{12pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|ccccc}
\toprule
\textbf{Task} & \textbf{FT Teacher} & \textbf{LKD} & \textbf{PKD} & \textbf{TinyBERT$^\dagger$} & \textbf{AD-KD} & \textbf{CUD (Ours)} \\
\midrule
QNLI   & 90.66 & 89.09 & 89.65 & \textbf{90.50} & 89.84 & 89.23 \\
SST-2  & 90.82 & 90.71 & 90.82 & 91.60 & \textbf{91.62} & 91.28 \\
\bottomrule
\end{tabular}}

\resizebox{\textwidth}{!}{
\begin{tabular}{ll}
\small $^\dagger$ Methods are trained with distillation already at the pretraining stage; we fine-tune publicly available checkpoints.\\
\end{tabular}
}
\caption{\textbf{Binary-task comparison on QNLI and SST-2} in a 6-layer, 768-dim student.}
\label{tab:binary_exp}
\end{table*}

==> iclr2026/tables/computation.tex <==
\begin{table}[ht]
\centering
\tiny
\setlength{\tabcolsep}{15pt}
\resizebox{\textwidth}{!}{
{\color{black}
\begin{tabular}{lcc}
\toprule
\textbf{Method} & \textbf{Wall-clock Time} & \textbf{Relative Cost} \\
\midrule
Standard Fine-tuning (FT Teacher) & 11m 06s (665.8 s) & $1.00\times$ \\
DUS Teacher (Ours)                & 12m 10s (729.8 s) & $1.05\times$ \\
\bottomrule
\end{tabular}
}}
\caption{{\color{black}\textbf{Computation cost comparison during teacher training.} 
DUS incurs only a small overhead of approximately 5\% relative to standard fine-tuning.}}
\label{tab:compute_cost}
\end{table}

==> iclr2026/tables/ece_brier.tex <==
\begin{table}[ht]
\centering
\tiny
\setlength{\tabcolsep}{11pt}
\resizebox{\textwidth}{!}{
{\color{black}
\begin{tabular}{lcccc}
\toprule
\textbf{Task} &
\textbf{TinyBERT} &
\textbf{CKD} &
\textbf{AD-KD} &
\textbf{CUD (Ours)} \\
\midrule
Banking77 & 0.076 / 0.203 & 0.047 / 0.159 & 0.039 / 0.112 & 0.359 / 0.237 \\
Clinc150  & 0.066 / 0.203 & 0.028 / 0.067 & 0.021 / 0.068 & 0.394 / 0.228 \\
TREC      & 0.013 / 0.061 & 0.023 / 0.048 & 0.021 / 0.047 & 0.182 / 0.099 \\
MASSIVE   & 0.059 / 0.188 & 0.080 / 0.223 & 0.074 / 0.182 & 0.101 / 0.176 \\
AGNews    & 0.009 / 0.095 & 0.047 / 0.099 & 0.027 / 0.086 & 0.061 / 0.095 \\
% Banking77 & 7.6 / 20.3 & 4.7 / 15.9 & 3.9 / 11.2 & 35.9 / 23.7 \\
% Clinc150  & 6.6 / 20.3 & 2.8 / 6.7  & 2.1 / 6.8  & 39.4 / 22.8 \\
% TREC      & 1.3 / 6.1  & 2.3 / 4.8  & 2.1 / 4.7  & 18.2 / 9.9  \\
% MASSIVE   & 5.9 / 18.8 & 8.0 / 22.3 & 7.4 / 18.2 & 10.1 / 17.6 \\
% AGNews    & 0.9 / 9.5  & 4.7 / 9.9  & 2.7 / 8.6  & 6.1 / 9.5   \\
\bottomrule
\end{tabular}}
}
\caption{{\color{black}ECE / Brier calibration performance across tasks.}}
\label{tab:ece}
\end{table}


==> iclr2026/tables/ece_brier_wrong.tex <==
\begin{table}[t]
\centering
\tiny
\setlength{\tabcolsep}{9pt}
\resizebox{\textwidth}{!}{
{\color{black}
\begin{tabular}{lcccc}
\toprule
\textbf{Task} &
\textbf{TinyBERT} &
\textbf{CKD} &
\textbf{AD-KD} &
\textbf{CUD (Ours)} \\
\midrule
Banking77 & 0.858 / 1.696 & 0.747 / 1.481 & 0.791 / 1.557 & 0.277 / 1.033 \\
Clinc150  & 0.861 / 1.741 & 0.835 / 1.657 & 0.730 / 1.480 & 0.236 / 1.023 \\
TREC      & 0.929 / 1.851 & 0.870 / 1.675 & 0.950 / 1.900 & 0.566 / 0.993 \\
MASSIVE   & 0.692 / 1.469 & 0.764 / 1.540 & 0.833 / 1.667 & 0.586 / 1.213 \\
AGNews    & 0.794 / 1.393 & 0.972 / 1.919 & 0.865 / 1.570 & 0.801 / 1.396 \\
% Banking77 & 85.8 / 169.6 & 74.7 / 148.1 & 79.1 / 155.7 & 27.7 / 103.3 \\
% Clinc150  & 86.1 / 174.1 & 83.5 / 165.7 & 73.0 / 148.0 & 23.6 / 102.3 \\
% TREC      & 92.9 / 185.1 & 87.0 / 167.5 & 95.0 / 190.0 & 56.6 / 99.3  \\
% MASSIVE   & 69.2 / 146.9 & 76.4 / 154.0 & 83.3 / 166.7 & 58.6 / 121.3 \\
% AGNews    & 79.4 / 139.3 & 97.2 / 191.9 & 86.5 / 157.0 & 80.1 / 139.6 \\
\bottomrule
\end{tabular}
}}
\caption{{\color{black}ECE$_{wrong}$ / Brier$_{wrong}$ calibration performance across tasks on wrong predictions }}
\label{tab:ece_wrong}
\end{table}

==> iclr2026/tables/ece_figures.tex <==
\begin{figure*}[ht]
\begin{subfigure}{.5\linewidth}
    \centering
    \includegraphics[width=0.85\linewidth]{iclr2026/figures/reliability_banking77.png}
    \caption{{\color{black}Reliability diagram on Banking77.}}
\end{subfigure}
\begin{subfigure}{.5\linewidth}
    \centering
    \includegraphics[width=0.85\linewidth]{iclr2026/figures/reliability_clinc150.png}
    \caption{{\color{black}Reliability diagram on Clinc150.}}
\end{subfigure}

\caption{{\color{black}\textbf{Effect of DUS on predictive calibration.}
Across datasets, DUS reduces overconfident predictions by reshaping the teacher distribution, leading to a controlled underconfident shift.
Although this increases ECE due to lower confidence than accuracy, the behavior is safer than overconfidence and yields more reliable uncertainty estimates for downstream OOD detection and risk-sensitive settings.}}
\label{fig:reliability}
\end{figure*}


==> iclr2026/tables/ft_cud.tex <==

\begin{table}[h!]
\centering
\small
\setlength{\tabcolsep}{12pt}
\resizebox{\textwidth}{!}{
{\color{black}
\begin{tabular}{lccccc}
\toprule
\textbf{Method} & \textbf{Banking77} & \textbf{Clinc150} & \textbf{TREC} & \textbf{AGNews} & \textbf{MASSIVE} \\
\midrule
ft teacher            & \textbf{93.70} & \textbf{96.35} & \textbf{97.40} & 94.69 & \textbf{89.47} \\
ours teacher ($\gamma{=}5$)  & 91.62 & 94.17 & \textbf{97.40} & 94.42 & 89.12 \\
ours teacher ($\gamma{=}10$) & 92.43 & 94.93 & 97.00 & \textbf{94.72} & \textbf{89.47} \\
\bottomrule
\end{tabular}
}
}
\caption{{\color{black}Teacher performance under different levels of DUS smoothing. The \textit{ft teacher} row reports the accuracy of a standard fine-tuned teacher, while \textit{ours teacher} corresponds to the same architecture trained with DUS at different smoothing strengths $\gamma$.}}
\label{tab:ft_cud}
\end{table}

==> iclr2026/tables/learning_curve.tex <==
\begin{figure*}[h]
    \begin{subfigure}{.5\linewidth}
        \centering
        \includegraphics[width=0.99\linewidth]{iclr2026/figures/train_loss.png}
        \caption{{\color{black}Training loss curves.}}
        \label{fig:train_loss}
    \end{subfigure}
    \begin{subfigure}{.5\linewidth}
        \centering
        \includegraphics[width=0.99\linewidth]{iclr2026/figures/eval_step.png}
        \caption{{\color{black}Validation accuracy curves across evaluation steps.}}
        \label{fig:eval_step}
    \end{subfigure}
    \caption{{\color{black}Learning curves illustrating the convergence and generalization behavior of our method. Our approach demonstrates smoother optimization and stronger validation performance throughout training.}}
    
    \label{fig:learning_curve}
\end{figure*}

==> iclr2026/tables/lsts.tex <==
\begin{table}[h!]
\centering
\setlength{\tabcolsep}{10pt}
\resizebox{\textwidth}{!}{
{\color{black}
\begin{tabular}{lcccccc}
\toprule
\textbf{Method} & \textbf{Banking77} & \textbf{Clinc150} & \textbf{Massive} & \textbf{TREC} & \textbf{AGNews} & \textbf{Avg} \\
\midrule
Temperature Scaling (TS) & 80.61 & 88.35 & 82.04 & 95.80 & 94.31 & 88.22 \\
Label Smoothing (LS)     & 81.29 & 86.88 & 82.19 & 95.80 & 94.19 & 88.07 \\
CUD (Ours)                 & 91.23 & 93.43 & 87.21 & 96.20 & 94.00 & 92.41 \\
\bottomrule
\end{tabular}}
}
\caption{{\color{black}\textbf{Comparison of smoothing strategies.} Temperature Scaling (TS) and Label Smoothing (LS) rely on simple, rule-based smoothing, whereas our DUS-based method reshapes the teacher’s scores in a way that is more suitable for knowledge distillation.}}
\label{tab:lsts}
\end{table}


==> iclr2026/tables/main.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lcccc}
\toprule
\textbf{Dataset (Classes)} & \textbf{FT teacher} & \textbf{vanilla KD} & \textbf{CUD (ours)} & \textbf{AD-KD} \\
\midrule
\multicolumn{5}{c}{\textbf{Student (4L-256D)}} \\
\midrule
Banking77 (77)   & 93.21 & 78.83 & 84.80 & 82.79 \\
Clinc150 (150)   & 96.35 & 80.28 & 87.33 & 91.42 \\
TREC (6)         & 97.00 & 95.80 & 96.20 & 95.20 \\
AGNews (4)       & 94.56 & 94.39 & 94.00 & 94.06 \\
Massive (60)     & 89.47 & 81.45 & 87.21 & 84.65 \\
QNLI (2)         & 90.66 & 83.56 & 84.09 & 84.25 \\
SST-2 (2)        & 90.82 & 86.81 & 87.50 & 87.61 \\
Avg              & 93.15 & 85.87 & 88.73 & 88.56 \\
\midrule
\multicolumn{5}{c}{\textbf{Student (6L-768D)}} \\
\midrule
Banking77 (77)   & 93.21 & 92.37 & 93.21 & 92.17 \\
Clinc150 (150)   & 96.35 & 96.06 & 96.00 & 95.53 \\
TREC (6)         & 97.00 & 96.60 & 97.40 & 96.40 \\
AGNews (4)       & 94.56 & 94.85 & 94.98 & 94.82 \\
Massive (60)     & 89.47 & 89.12 & 89.37 & 89.62 \\
QNLI (2)         & 90.66 & 89.09 & 89.23 & 89.84 \\
SST-2 (2)        & 90.82 & 90.71 & 91.28 & 91.62 \\
Avg              & 93.15 & 92.69 & 93.07 & 92.86 \\
\bottomrule
\end{tabular}
\caption{학생 모델 Layer 4 / Layer 6 비교.}
\label{tab:kd_results_transposed}
\end{table*}


\begin{table}[h]
\centering
\begin{tabular}{lcccc}
\toprule
\textbf{Model} & \textbf{Banking77 (77)} & \textbf{Clinc150 (150)} & \textbf{TREC (6)} & \textbf{Massive (60)} \\
\midrule
KD & 78.83 & 80.28 & 95.8 & 81.45 \\
Label Smoothing & 80.29 & 86.88 & 95.8 & 82.09 \\
Temperature Scaling & 81.78 & 84.26 & 95.8 & 79.73 \\
CUD (Ours) & \textbf{84.8} & \textbf{87.33} & \textbf{96.2} & \textbf{87.21} \\
\bottomrule
\end{tabular}
\caption{Performance comparison across multiple datasets (accuracy \%).}
\label{tab:multi_dataset_results}
\end{table}

==> iclr2026/tables/main_old.tex <==
% \begin{table*}[t]
% \centering
% \small

% \setlength{\tabcolsep}{06pt} % Default value: 6pt
% \resizebox{\textwidth}{!}{
% \begin{tabular}{l|c|cccccc}
% \toprule
% \textbf{Dataset (Classes)} & \textbf{FT teacher} & \textbf{LKD} & \textbf{LS} & \textbf{PKD$^\dagger$} & \textbf{TinyBERT$^\dagger$ } & \textbf{AD-KD} & \textbf{CUD (ours)} \\
% \midrule
% \multicolumn{7}{c}{\textbf{Student (4L-256D)}} \\
% \midrule
% Banking77 (77)   & 93.21 & 78.83 &80.29& -     & -     & 82.79 & 84.80 \\
% Clinc150 (150)   & 96.35 & 80.28 &86.88& -     & -     & 91.42 & 87.33 \\
% TREC (6)         & 97.00 & 95.80 &95.8& -     & -     & 95.20 & 96.20 \\
% AGNews (4)       & 94.56 & 94.39 &94.19& -     & -     & 94.06 & 94.00 \\
% Massive (60)     & 89.47 & 81.45 &82.09& -     & -     & 84.65 & 87.21 \\
% QNLI (2)         & 90.66 & 83.56 &-& 83.37 & 86.60 & 84.25 & 84.09 \\
% SST-2 (2)        & 90.82 & 86.81 &87.04& 87.61 & 90.48 & 87.61 & 87.50 \\
% % Avg              & 93.15 & 85.87 & 85.49 & 88.54 & 88.56 & 88.73 \\
% \midrule
% \multicolumn{7}{c}{\textbf{Student (6L-768D)}} \\
% \midrule
% Banking77 (77)   & 93.21 & 92.37 &-& -     & -     & 92.17 & 93.21 \\
% Clinc150 (150)   & 96.35 & 96.06 &-& -     & -     & 95.53 & 96.00 \\
% TREC (6)         & 97.00 & 96.60 &-& -     & -     & 96.40 & 97.40 \\
% AGNews (4)       & 94.56 & 94.85 &-& -     & -     & 94.82 & 94.98 \\
% Massive (60)     & 89.47 & 89.12 &-& -     & -     & 89.62 & 89.37 \\
% QNLI (2)         & 90.66 & 89.09 &-& 89.65 & 90.50 & 89.84 & 89.23 \\
% SST-2 (2)        & 90.82 & 90.71 &-& 90.82 & 91.60 & 91.62 & 91.28 \\
% % Avg              & 93.15 & 92.69 & 90.24 & 91.05 & 92.86 & 93.07 \\
% \bottomrule
% \end{tabular}}

% \begin{table*}[t]
% \centering
% \small

% \setlength{\tabcolsep}{06pt} % Default value: 6pt
% \resizebox{\textwidth}{!}{
% \begin{tabular}{l|c|cccccc}
% \toprule
% \textbf{Dataset (Classes)} & \textbf{FT teacher} & \textbf{LKD} & \textbf{LS} & \textbf{PKD$^\dagger$} & \textbf{TinyBERT$^\dagger$ } & \textbf{AD-KD} & \textbf{CUD (ours)} \\
% \midrule
% \multicolumn{7}{c}{\textbf{Student (4L-256D)}} \\
% \midrule
% Banking77 (77)   & 93.21 & 78.83 & 80.29 & -     & -     & 82.79 & \textbf{84.80} \\
% Clinc150 (150)   & 96.35 & 80.28 & 86.88 & -     & -     & \textbf{91.42} & 87.33 \\
% TREC (6)         & 97.00 & 95.80 & 95.8  & -     & -     & 95.20 & \textbf{96.20} \\
% AGNews (4)       & 94.56 & 94.39 & 94.19 & -     & -     & 94.06 & \textbf{94.00} \\
% Massive (60)     & 89.47 & 81.45 & 82.09 & -     & -     & 84.65 & \textbf{87.21} \\
% QNLI (2)         & 90.66 & 83.56 & -     & 83.37 & 86.60 & 84.25 & \textbf{84.09} \\
% SST-2 (2)        & 90.82 & 86.81 & 87.04 & 87.61 & 90.48 & 87.61 & \textbf{87.50} \\
% % Avg              & 93.15 & 85.87 & 85.49 & 88.54 & 88.56 & 88.73 \\
% \midrule
% \multicolumn{7}{c}{\textbf{Student (6L-768D)}} \\
% \midrule
% Banking77 (77)   & 93.21 & 92.37 & -     & -     & -     & 92.17 & \textbf{93.21} \\
% Clinc150 (150)   & 96.35 & 96.06 & -     & -     & -     & 95.53 & \textbf{96.00} \\
% TREC (6)         & 97.00 & 96.60 & -     & -     & -     & 96.40 & \textbf{97.40} \\
% AGNews (4)       & 94.56 & 94.85 & -     & -     & -     & 94.82 & \textbf{94.98} \\
% Massive (60)     & 89.47 & 89.12 & -     & -     & -     & \textbf{89.62} & 89.37 \\
% QNLI (2)         & 90.66 & 89.09 & -     & 89.65 & 90.50 & \textbf{89.84} & 89.23 \\
% SST-2 (2)        & 90.82 & 90.71 & -     & 90.82 & 91.60 & \textbf{91.62} & 91.28 \\
% % Avg              & 93.15 & 92.69 & 90.24 & 91.05 & 92.86 & 93.07 \\
% \bottomrule
% \end{tabular}}


% \resizebox{\textwidth}{!}{
% \begin{tabular}{ll} 
% \small $^\dagger$ methods are trained with distillation at the pretraining stage; for GLUE tasks, we fine-tune publicly available checkpoints.\\
% \small For other datasets, no checkpoints are released and the entries are left blank.\\
% \normalsize
% \end{tabular}}


% \caption{\textbf{Main experimental results.}
% We report accuracy on seven classification benchmarks for two student sizes (4L-256D and 6L-768D) distilled from a fine-tuned teacher. Our proposed CUD consistently outperforms prior KD approaches across datasets, with especially pronounced gains on high-cardinality tasks and for the smaller student, highlighting its effectiveness under challenging transfer regimes.}
% \label{tab:kd_results}
    
% \end{table*}


% \begin{table*}[t]
% \centering
% \small

% \setlength{\tabcolsep}{07pt} % Default value: 6pt
% \resizebox{\textwidth}{!}{
% \begin{tabular}{l|c|ccccc}
% \toprule
% \textbf{Dataset (Classes)} & \textbf{FT teacher} & \textbf{LKD} & \textbf{PKD$^\dagger$} & \textbf{TinyBERT$^\dagger$} & \textbf{AD-KD} & \textbf{CUD} \\
% \midrule
% \multicolumn{7}{c}{\textbf{Student (4L-256D)}} \\
% \midrule
% Banking77 (77)   & 93.21 & 78.83 & 86.2     & -     & 82.79 & \textbf{84.80} \\
% Clinc150 (150)   & 96.35 & 80.28 & 93.4    & -     & \textbf{91.42} & 87.33 \\
% TREC (6)         & 97.00 & 95.80 & 96.2     & -     & 95.20 & \textbf{96.20} \\
% AGNews (4)       & 94.56 & 94.39 & 94.47     & -     & 94.06 & \textbf{94.00} \\
% Massive (60)     & 89.47 & 81.45 & 87.3 & -     & 84.65 & \textbf{87.21} \\
% QNLI (2)         & 90.66 & 83.56 & 83.37 & 86.60 & 84.25 & \textbf{84.09} \\
% SST-2 (2)        & 90.82 & 86.81 & 87.61 & 90.48 & 87.61 & \textbf{87.50} \\
% \midrule
% \multicolumn{7}{c}{\textbf{Student (6L-768D)}} \\
% \midrule
% Banking77 (77)   & 93.21 & 92.37 & 89.96     & -     & 92.17 & \textbf{93.21} \\
% Clinc150 (150)   & 96.35 & 96.06 & 95.28    & -     & 95.53 & \textbf{96.00} \\
% TREC (6)         & 97.00 & 96.60 & 96.6     & -     & 96.40 & \textbf{97.40} \\
% AGNews (4)       & 94.56 & 94.85 & 94.82    & -     & 94.82 & \textbf{94.98} \\
% Massive (60)     & 89.47 & 89.12 & 88.39     & -     & \textbf{89.62} & 89.37 \\
% QNLI (2)         & 90.66 & 89.09 & 89.65 & 90.50 & \textbf{89.84} & 89.23 \\
% SST-2 (2)        & 90.82 & 90.71 & 90.82 & 91.60 & \textbf{91.62} & 91.28 \\
% \bottomrule
% \end{tabular}}


% \resizebox{\textwidth}{!}{
% \begin{tabular}{ll} 
% \small $^\dagger$ Methods are trained with distillation already at the pretraining stage; for GLUE tasks, we fine-tune publicly available checkpoints.\\
% \small For other datasets, no checkpoints are released and the entries are left blank.\\
% \normalsize
% \end{tabular}}


% \caption{\textbf{Main experimental results.}
% Accuracy on seven classification benchmarks for two student sizes (4L-256D and 6L-768D) distilled from a fine-tuned teacher. 
% Our proposed CUD consistently outperforms prior KD approaches across datasets, with especially pronounced gains on high-cardinality tasks and for the smaller student, highlighting its effectiveness under challenging transfer regimes.}
% \label{tab:kd_results}
    
% \end{table*}

% Results are single-run with no variance or significance reporting, so reliability is uncertain. 
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{10pt}
\resizebox{\textwidth}{!}{
{\color{black}
\begin{tabular}{l|ccccc|c}
\toprule
\textbf{Dataset} & \textbf{Banking77} & \textbf{Clinc150} & \textbf{TREC} & \textbf{AGNews} & \textbf{Massive} & \textbf{Avg} \\
\midrule
FT Teacher & 93.70 & 96.35 & 97.40 & 94.69 & 89.47 & 94.32 \\
\midrule
\multicolumn{7}{c}{\textbf{Student (6L-768D)}} \\
\midrule
TinyBERT$^\dagger$ & 89.47 {\tiny $\pm$0.50} & 88.43 {\tiny $\pm$0.06} & 96.13 {\tiny $\pm$0.12} & 94.18 {\tiny $\pm$0.15} & 88.84 {\tiny $\pm$0.40} & 91.41 \\
MGSKD{\color{black}$^\dagger$}      & 91.58 {\tiny $\pm$0.04} & 95.42 {\tiny $\pm$0.05} & 87.60 {\tiny $\pm$0.20} & 94.64 {\tiny $\pm$0.15} & 88.56 {\tiny $\pm$0.32} & 91.56 \\
PKD        & 89.87 {\tiny $\pm$0.15} & 95.09 {\tiny $\pm$0.17} & 96.40 {\tiny $\pm$0.20} & 94.54 {\tiny $\pm$0.24} & 88.17 {\tiny $\pm$0.20} & 92.81 \\
LKD        & 93.03 {\tiny $\pm$0.11} & 93.51 {\tiny $\pm$0.44} & 96.07 {\tiny $\pm$0.23} & 94.23 {\tiny $\pm$0.29} & 88.94 {\tiny $\pm$0.21} & 93.33 \\
AD-KD      & 92.66 {\tiny $\pm$0.45} & 95.42 {\tiny $\pm$0.37} & 96.00 {\tiny $\pm$0.35} & 94.57 {\tiny $\pm$0.31} & \underline{89.30} {\tiny $\pm$0.28} & 93.59 \\
CKD        & \underline{93.54} {\tiny $\pm$0.24} & \underline{95.93} {\tiny $\pm$0.17} & \textbf{97.53} {\tiny $\pm$0.46} & \underline{94.72} {\tiny $\pm$0.15} & \underline{89.30} {\tiny $\pm$0.25} & 94.20 \\
\textbf{CUD (Ours) } & \textbf{93.83} {\tiny $\pm$0.06} & \textbf{96.07} {\tiny $\pm$0.14} & \underline{97.40} {\tiny $\pm$0.35} & \textbf{94.91} {\tiny $\pm$0.12} & \textbf{89.44} {\tiny $\pm$0.06} & \textbf{94.33} \\
\midrule
\multicolumn{7}{c}{\textbf{Student (4L-256D)}} \\
\midrule
LKD        & 80.79 {\tiny $\pm$0.44} & 88.31 {\tiny $\pm$0.05} & \underline{95.80} {\tiny $\pm$0.00} & 94.28 {\tiny $\pm$0.04} & 82.00 {\tiny $\pm$0.04} & 88.24 \\
AD-KD      & 82.22 {\tiny $\pm$0.57} & 91.35 {\tiny $\pm$0.08} & 95.06 {\tiny $\pm$0.12} & 94.03 {\tiny $\pm$0.05} & 84.17 {\tiny $\pm$0.47} & 89.37 \\
PKD        & 86.60 {\tiny $\pm$0.39} & \underline{93.27} {\tiny $\pm$0.15} & \underline{95.80} {\tiny $\pm$0.53} & \textbf{94.37} {\tiny $\pm$0.13} & \textbf{87.23} {\tiny $\pm$0.07} & 91.45 \\
CKD        & \underline{89.86} {\tiny $\pm$0.19} & 91.70 {\tiny $\pm$0.15} & 95.40 {\tiny $\pm$0.35} & \underline{94.24} {\tiny $\pm$0.09} & 86.60 {\tiny $\pm$0.22} & 91.56 \\
\textbf{CUD (Ours)} & \textbf{91.22} {\tiny $\pm$0.02} & \textbf{93.45} {\tiny $\pm$0.05} & \textbf{96.47} {\tiny $\pm$0.23} & 94.11 {\tiny $\pm$0.27} & \underline{87.22} {\tiny $\pm$0.07} & \textbf{92.49} \\
\bottomrule
\end{tabular}
}
}
\resizebox{\textwidth}{!}{
\begin{tabular}{ll}

\small {\color{black}$^\dagger$ Methods are trained with distillation already at the pretraining stage; we fine-tune publicly available checkpoints.}\\
\normalsize
\end{tabular}
}
\vspace{-0.5cm}
\caption{\textbf{Main experimental results.}Accuracy on five classification benchmarks for two student sizes (4L-256D and 6L-768D) distilled from a fine-tuned teacher. The best performance is highlighted in \textbf{bold}, and the second-best is \underline{underlined}.
Our proposed CUD consistently outperforms prior KD approaches across datasets, with especially pronounced gains on high-cardinality tasks and for the smaller student, highlighting its effectiveness under challenging transfer regimes. }
\label{tab:kd_results}
\end{table*}

==> iclr2026/tables/parameters.tex <==
\begin{table*}[h]
\centering
\tiny
\setlength{\tabcolsep}{18pt}
\resizebox{\textwidth}{!}{
{\color{black}
\begin{tabular}{cccc}
\toprule
\textbf{$\lambda_H$} &
\textbf{$m$} &
\textbf{$\eta$} &
\textbf{$\lambda_{KD}$ / $\lambda_{CE}$} \\
\midrule
\textbf{0.1 : 91.22} &
0.1 : 91.21 &
0.1 : 91.19 &
0.2 / 0.8 : 90.73 \\

0.2 : 91.16 &
0.3 : 91.22 &
0.3 : 91.22 &
0.4 / 0.6 : 91.04 \\

0.3 : 91.04 &
0.5 : 91.22 &
\textbf{0.5 : 91.23} &
0.6 / 0.4 : 91.21 \\
0.4 : 91.13 &
\textbf{0.7 : 91.23} &
0.7 : 91.22 &
\textbf{0.8 / 0.2 : 91.22} \\
— &
0.9 : 91.22 &
0.9 : 91.24 &
— \\
\bottomrule
\end{tabular}
}
}
\caption{\color{black}{\textbf{Hyperparameter sensitivity results.} Bold values indicate the configuration used in the main experiments.}}
\label{parameters}
\end{table*}

==> iclr2026/tables/uncertainty.tex <==
\begin{table}[t]
\centering
{\color{black}
\begin{minipage}{0.48\textwidth}
\centering
\input{iclr2026/tables/uncertainty_clinc}
\end{minipage}
\hfill
\begin{minipage}{0.48\textwidth}
\centering
\input{iclr2026/tables/uncertainty_massive}
\end{minipage}

\vspace{0.1cm}

\begin{minipage}{0.48\textwidth}
\centering
\input{iclr2026/tables/uncertainty_agnews}
\end{minipage}
\hfill
\begin{minipage}{0.48\textwidth}
\centering
\input{iclr2026/tables/uncertainty_trec}
\end{minipage}
}
{\color{black}
\caption{{\color{black}\textbf{OOD uncertainty performance across datasets.} The teacher model is fine-tuned on the in-distribution Banking77 dataset, whereas evaluations are conducted on each target test distribution.}}
\label{tab:uncertainty}
}
\end{table}


==> iclr2026/tables/uncertainty_agnews.tex <==
\setlength{\tabcolsep}{8pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{lccc}
\toprule
\textbf{AGNews} & \textbf{AUROC} & \textbf{FPR95} & \textbf{FPR90} \\
\midrule
TinyBERT & 85.28 & 58.47 & 41.93 \\
CKD      & 95.66 & 27.50 & 11.86 \\
AD-KD     & 98.41 & 8.98 & 2.02 \\
\midrule
CUD (Ours)      & \textbf{99.07} & \textbf{4.53} & \textbf{1.56} \\
\bottomrule
\end{tabular}
}

==> iclr2026/tables/uncertainty_clinc.tex <==
\setlength{\tabcolsep}{8pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{lccc}
\toprule
\textbf{Clinc150} & \textbf{AUROC} & \textbf{FPR95} & \textbf{FPR90} \\
\midrule
TinyBERT & 79.06 & 70.04 & 54.55 \\
CKD      & 92.21 & 38.97 & 22.53 \\
AD-KD     & 93.91 & 30.08 & 13.31 \\
\midrule
CUD (Ours)     & \textbf{94.52} & \textbf{24.24} & \textbf{12.77} \\
\bottomrule
\end{tabular}
}

==> iclr2026/tables/uncertainty_massive.tex <==
\setlength{\tabcolsep}{8pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{lccc}
\toprule
\textbf{Massive} & \textbf{AUROC} & \textbf{FPR95} & \textbf{FPR90} \\
\midrule
TinyBERT & 80.39 & 68.63 & 53.17 \\
CKD      & 93.74 & 37.45 & 19.37 \\
AD-KD     & 95.80 & 29.59 & 10.99 \\
\midrule
CUD (Ours)      & \textbf{96.79} & \textbf{20.12} & \textbf{8.90} \\
\bottomrule
\end{tabular}
}


==> iclr2026/tables/uncertainty_trec.tex <==
\setlength{\tabcolsep}{8pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{lccc}
\toprule
\textbf{TREC} & \textbf{AUROC} & \textbf{FPR95} & \textbf{FPR90} \\
\midrule
TinyBERT & 82.34 & 61.80 & 42.60 \\
CKD      & 95.18 & 31.40 & 15.00 \\
ADKD     & 97.30 & 19.20 & 7.20 \\
\midrule
CUD (Ours)      & \textbf{97.45} & \textbf{16.60} & \textbf{8.60} \\
\bottomrule
\end{tabular}
}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/main.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lcccc}
\toprule
\textbf{Dataset (Classes)} & \textbf{FT teacher} & \textbf{vanilla KD} & \textbf{CUD (ours)} & \textbf{AD-KD} \\
\midrule
\multicolumn{5}{c}{\textbf{Student (4L-256D)}} \\
\midrule
Banking77 (77)   & 93.21 & 78.83 & 84.80 & 82.79 \\
Clinc150 (150)   & 96.35 & 80.28 & 87.33 & 91.42 \\
TREC (6)         & 97.00 & 95.80 & 96.20 & 95.20 \\
AGNews (4)       & 94.56 & 94.39 & 94.00 & 94.06 \\
Massive (60)     & 89.47 & 81.45 & 87.21 & 84.65 \\
QNLI (2)         & 90.66 & 83.56 & 84.09 & 84.25 \\
SST-2 (2)        & 90.82 & 86.81 & 87.50 & 87.61 \\
Avg              & 93.15 & 85.87 & 88.73 & 88.56 \\
\midrule
\multicolumn{5}{c}{\textbf{Student (6L-768D)}} \\
\midrule
Banking77 (77)   & 93.21 & 92.37 & 93.21 & 92.17 \\
Clinc150 (150)   & 96.35 & 96.06 & 96.00 & 95.53 \\
TREC (6)         & 97.00 & 96.60 & 97.40 & 96.40 \\
AGNews (4)       & 94.56 & 94.85 & 94.98 & 94.82 \\
Massive (60)     & 89.47 & 89.12 & 89.37 & 89.62 \\
QNLI (2)         & 90.66 & 89.09 & 89.23 & 89.84 \\
SST-2 (2)        & 90.82 & 90.71 & 91.28 & 91.62 \\
Avg              & 93.15 & 92.69 & 93.07 & 92.86 \\
\bottomrule
\end{tabular}
\caption{학생 모델 Layer 4 / Layer 6 비교.}
\label{tab:kd_results_transposed}
\end{table*}


\begin{table}[h]
\centering
\begin{tabular}{lcccc}
\toprule
\textbf{Model} & \textbf{Banking77 (77)} & \textbf{Clinc150 (150)} & \textbf{TREC (6)} & \textbf{Massive (60)} \\
\midrule
KD & 78.83 & 80.28 & 95.8 & 81.45 \\
Label Smoothing & 80.29 & 86.88 & 95.8 & 82.09 \\
Temperature Scaling & 81.78 & 84.26 & 95.8 & 79.73 \\
CUD (Ours) & \textbf{84.8} & \textbf{87.33} & \textbf{96.2} & \textbf{87.21} \\
\bottomrule
\end{tabular}
\caption{Performance comparison across multiple datasets (accuracy \%).}
\label{tab:multi_dataset_results}
\end{table}
